Ferromagnetic Ising Model on multiregular random graphs

A family of multispecies Ising models on generalized regular random graphs is investigated in the thermodynamic limit. The architecture is specified by class-dependent couplings and magnetic fields. We prove that the magnetizations, neighbours correlations and free energy converge to suitable functions evaluated at the solution of a belief propagation fixed point equation. In absence of magnetic fields, a phase transition is identified and the corresponding critical parameters are determined by the spectral radius of a low-dimensional matrix.

==> Free_energy/lemma_analysis.tex <==
\begin{lemma}
    Given $f(\mathbf{x})$, $g(\mathbf{x})$ both $\mathrm{R}^{n+}\rightarrow \mathrm{R}$, if $f(\mathbf{0})=g(\mathbf{0})$ and $\forall \; i=1,...,n$
    \begin{equation}
        \frac{\partial f(\mathbf{x})}{\partial x_i} = \frac{\partial g(\mathbf{x})}{\partial x_i} \quad \forall \; \mathbf{x}\in \mathrm{R}^{n+}
    \end{equation} 
    then 
    \begin{equation}
         f(\mathbf{x}) = g(\mathbf{x}) \quad \forall \; \mathbf{x}\in \mathrm{R}^{n+}
    \label{eq_lemma_analysis}
    \end{equation}
    \label{lemma_analysis}
\end{lemma}

\begin{proof}
    To prove that $f(\mathbf{x}) = g(\mathbf{x})$, for any $\mathbf{x}\in \mathrm{R}^{n+}$ we draw a segment with extremes $\mathbf{0}$ and $\mathbf{x}$, which is always inside the domain; the segment is parametrized by $s(t) = t\mathbf{x}$, $t\in(0,1]$. We can thus define the one-variable functions
    \begin{align}
        &\Tilde{f}(t) = f(t\mathbf{x}) \\
        &\Tilde{g}(t) = g(t\mathbf{x}) 
    \end{align}
    which by the fundamental theorem of calculus we can rewrite as 
    \begin{align}
        &\Tilde{f}(t) =  \Tilde{f}(0) +  \int_{0}^{t} \frac{\partial \Tilde{f}(t')}{\partial t'} dt' = f(\mathbf{0}) +  \int_{0}^{t} <\mathbf{\nabla}f(t'\mathbf{x}),\mathbf{x}> dt'  \\
        &\Tilde{g}(t) =  \Tilde{g}(0) +  \int_{0}^{t} \frac{\partial \Tilde{g}(t')}{\partial t'} dt' = g(\mathbf{0}) +  \int_{0}^{t} <\mathbf{\nabla}g(t'\mathbf{x}),\mathbf{x}> dt'
    \end{align}
    where in the second equalities we applied the chain rule. As $f(\mathbf{0})=g(\mathbf{0})$ and $\mathbf{\nabla}f(\mathbf{y})=\mathbf{\nabla}g(\mathbf{y})$ $\forall \; \mathbf{y}\in \mathrm{R}^{n+}$ by hypothesis, and since $f(\mathbf{x})=\Tilde{f}(1)$,$g(\mathbf{x})=\Tilde{g}(1)$, we have (\ref{eq_lemma_analysis}).
\end{proof}


==> Free_energy/theo_bethe_free_en.tex <==
The next theorem proves that for all non-negative fields, the free energy of the model converges in the thermodynamic limit to the Bethe free energy calculated at the unique fixed point of the recursion reached with non-negative initialization. \\
\\
The Bethe free energy calculated at the messages (or cavity fields) of the Belief Propagation algorithm is typically used as an approximation for the free energy of the model: whenever there are multiple fixed point of the BP algorithm, the heuristics prescribe to take the Bethe free energy calculated at the fixed point for which it is minimum. The derived exact recursion corresponds to the BP equations with the symmetry constraint $h^*_{i\rightarrow j} = h^*_{C_a\rightarrow C_b}, \; \forall \; i\in C_a, j\in C_b$ (the messages after convergence depend only on the classes of the extremes). We basically proved that the BP algorithm for the ferromagnetic Ising model on $\mathbf{k}$-regular random graphs with non-negative fields has a least one solution constrained to $h_{i\rightarrow j} = h_{C_a\rightarrow C_b}, \; \forall \; i\in C_a, j\in C_b$, the fixed point with all positive entries under such constrain is unique and reached from any positive initialization, and the Bethe free energy calculated at that fixed point is the exact free energy of the model. 

\begin{theorem}
    Consider an Ising model on a $\boldsymbol{k}$-regular graph with $n$ classes, non-negative couplings and fields. The following limit exists and 
    \begin{equation}
        N^{-1}\log Z_N      \quad \xrightarrow[N\rightarrow \infty]{\Pprob} \quad       p(\boldsymbol{\beta},\boldsymbol{h})
    \label{eq_free_en_convergence}
    \end{equation}
    where
    \begin{align}
        p(\boldsymbol{\beta},\boldsymbol{h})& = \frac{1}{2} \sum_{a=1}^n \alpha_a \sum_{a'=1}^n k_{aa'} \bigg[ -\frac{1}{2}\log(1-\theta_{aa'}^2) - \log(1+\theta_{aa'}\tanh(\bar{z}_a^{(a')})\tanh(\bar{z}_{a'}^{(a)}))\bigg] \nonumber \\ 
        &+ \sum_{a=1}^n \alpha_a \log\bigg(e^{h_a} \prod_{a'=1}^n [1+\theta_{aa'}\tanh(\bar{z}_{a'}^{(a)})]^{k_{aa'}} + e^{-h_a} \prod_{a'=1}^n [1-\theta_{aa'}\tanh(\bar{z}_{a'}^{(a)})]^{k_{aa'}}\bigg)
        \label{free_energy}
    \end{align}
    where $\alpha_a = \frac{N_{C_a}}{N}, \; \forall a=1,...,n$ is the ratio of spins of class $a$ over the total size of the system and $\theta_{aa'}= \tanh(\beta_{aa'})$. 
\end{theorem}
\vskip 1 cm
\begin{proof}
    The proof proceeds in multiple steps:
    \begin{enumerate}[]
        \item Once defined $p_N(\boldsymbol{\beta},\boldsymbol{h})= N^{-1}\log Z_N$, we first show that $\forall\; N\in \mathbb{N}\;$ $p_N(\boldsymbol{0},\boldsymbol{h})= p(\boldsymbol{0},\boldsymbol{h})$

      
        \item We show that
        \begin{equation}
             \frac{1}{N} \sum_{<ij>\in E, i\in C_a, j\in C_{a'}} <\sigma_i \sigma_j>_{G_N}  \quad \xrightarrow[N\rightarrow \infty]{\Pprob} \frac{\alpha_a k_{aa'}}{2^{\delta_{aa'}}}<\sigma_1 \sigma_2>_{G',\mu'}  \quad\quad \forall \; a,a'=1,...,n 
        \label{eq_edge_covergence}
        \end{equation}
        where $G'(V,E)$, $V= \{i,j\}, E=\{ij\}$ and $\mu'$ is the Ising measure on such graph composed by a single edge, with coupling $\beta_{aa'}$ and fields $h'_a = \bar{z}_a^{(a')}$, $h'_{a'} = \bar{z}_{a'}^{(a)}$. $\delta_{aa'}$ is the Kronecker delta.

        \item We also show that 
        \begin{equation}
             \frac{\partial p(\boldsymbol{\beta},\boldsymbol{h})}{\partial \beta_{aa'}} =   \frac{\alpha_a k_{aa'}}{2^{\delta_{aa'}}}<\sigma_1 \sigma_2>_{G',\mu'}  \quad\quad \forall \; a,a'=1,...,n 
        \label{derivative_functional}
        \end{equation}
        
        \item Putting together the previous results, we have the convergence in probability of the derivatives
        \begin{equation}
            \frac{\partial p_N(\boldsymbol{\beta},\boldsymbol{h})}{\partial \beta_{aa'}} = \frac{1}{N} \sum_{<ij>\in E, i\in C_a, j\in C_{a'}} <\sigma_i \sigma_j>_{G_N}  \quad \xrightarrow[N\rightarrow \infty]{\Pprob} \frac{\partial p(\boldsymbol{\beta},\boldsymbol{h})}{\partial \beta_{aa'}}   \quad \quad \forall \; a,a'=1,...,n
        \end{equation}
        and the equivalence at one point. We show that the derivatives are also bounded and prove (\ref{eq_free_en_convergence}) by dominated convergence.
    \end{enumerate}
    \vskip 2 cm

    \begin{enumerate}[label=\textit{\arabic*}.]
        \item For the proof of the first point it suffices to compute the partition function in the non-interacting case
        \begin{equation}
            Z_N(\boldsymbol{0},\boldsymbol{h}) = \sum_{\boldsymbol{\sigma}}e^{\sum_{a=1}^nh_a\sum_{i\in C_a}\sigma_i} = \sum_{\boldsymbol{\sigma}} \prod_{a=1}^n \prod_{i\in C_a} e^{-h_a\sigma_i} = \prod_{a=1}^n [2\cosh{(h_a)}]^{N\alpha_a}
        \end{equation}
        from which we have 
        \begin{equation}
            p_N(\boldsymbol{0},\boldsymbol{h})= N^{-1}\log Z_N(\boldsymbol{0},\boldsymbol{h}) = \log(2) + \sum_{a=1}^n \alpha_a \log(\cosh{(h_a)}) = p(\boldsymbol{0},\boldsymbol{h})
        \end{equation}
        where the latter equality can be easily verified subsituting $\boldsymbol{\beta}=\boldsymbol{0}$ in (\ref{free_energy}).
        \vskip 0.8 cm

        \item By the GKS inequalities, $\forall i,j:<ij>\in E$, taking w.l.o.g. $i\in C_a,\; j\in C_{a'}$
        \begin{equation}
            <\sigma_i\sigma_j>_{T_{ij}(t)}^{\boldsymbol{0}} \quad \leq \quad <\sigma_i\sigma_j>_{G_N} \quad \leq \quad <\sigma_i\sigma_j>_{T_{ij}(t)}^{\boldsymbol{+}}
        \end{equation}
        where $T_{ij}(t)$ is a $\boldsymbol{k}$-regular tree centered in the edge $<ij>$, in the sense that the border is $t$ edges far from $<ij>$.  $\boldsymbol{0}$ and $\boldsymbol{+}$ refer, as usual, for respectively free and plus boundary conditions. If we manage to prove that 
         \begin{equation}
             <\sigma_i\sigma_j>_{T_{ij}(t)}^{\boldsymbol{0}}  \Nearrow \;<\sigma_1 \sigma_{2}>_{G',\mu'}  \;\;\;\;\;\;\;  <\sigma_i\sigma_j>_{T_{ij}(t)}^{\boldsymbol{+}} \Searrow \; <\sigma_1 \sigma_{2}>_{G',\mu'}  \;\;\;\;\;\;\; \mbox{for}\;t\rightarrow \infty
         \label{converg_eq}
         \end{equation}
        once noticed that for any $i\in C_a,\; j\in C_{a'}$ such trees are isomorphic, we could conclude, following the very same procedure of Lemma \ref{th_positive_fields_magnetization}, that 
        \begin{equation}
             <\sigma_i \sigma_j>_{G_N}  \quad \xrightarrow[N\rightarrow \infty]{\Pprob}  \quad <\sigma_1 \sigma_2>_{G',\mu'}  \;\;\;\;\;\;\; \forall \;i\in C_a,\; j\in C_{a'}
        \end{equation}
        Eventually, considering that there are $\alpha_a k_{aa'}$ edges of this type if $a\neq a'$, and $\frac{\alpha_a k_{aa'}}{2}$ edges of this type if $a= a'$, we would get (\ref{eq_edge_covergence}).\\
        For proving (\ref{converg_eq}) we use a similar technique of Lemma \ref{} and the same notation: exploiting the tree structure, we can split the Hamiltonian into two disjoint sides connected by the edge $<ij>$
        $$H = H_{T_i} + H_{T_j} + \beta_{aa'}\sigma_i \sigma_j$$
        \begin{align}  
            S_{ij,T_{ij}}(1) :&= \mu(\sigma_i\sigma_j) = \frac{\sum_{\boldsymbol{\sigma}: \sigma_i\sigma_j=1}e^{H_{T_i}+H_{T_j}+\beta_{aa'}\sigma_i\sigma_j}}{Z} = \frac{e^{\beta_{aa'}}}{Z} \sum_{\boldsymbol{\sigma}: \sigma_i\sigma_j=1} e^{H_{T_i}+H_{T_j}} =\\
            & = e^{\beta_{aa'}} \bigg[ \sum_{\boldsymbol{\sigma}: \sigma_i=1,\sigma_j=1} \frac{e^{H_{T_i}+H_{T_j}}}{Z} + \sum_{\boldsymbol{\sigma}: \sigma_i=-1,\sigma_j=-1} \frac{e^{H_{T_i}+H_{T_j}}}{Z} \bigg] =\\
            &= e^{\beta_{aa'}} \frac{Z_{T_i}Z_{T_j}}{Z} [S_{i,T_i}(1)S_{j,T_j}(1)+S_{i,T_i}(-1)S_{j,T_j}(-1)]
        \end{align}
        and in the same way 
        $$S_{ij,T_{ij}}(-1) = e^{-\beta_{aa'}} \frac{Z_{T_i}Z_{T_j}}{Z} [S_{i,T_i}(1)S_{j,T_j}(-1)+S_{i,T_i}(-1)S_{j,T_j}(1)]$$
        taking the ratio
        \begin{align}
            \frac{S_{ij,T_{ij}}(1)}{S_{ij,T_{ij}}(-1)} &= \frac{1+ <\sigma_i\sigma_j>}{1- <\sigma_i\sigma_j>} = e^{2\beta_{aa'}}  \frac{(1+\Tilde{m}_i^{(j)}) (1+\Tilde{m}_j^{(i)}) + (1-\Tilde{m}_i^{(j)})  (1-\Tilde{m}_j^{(i)}) }{(1+\Tilde{m}_i^{(j)}) (1-\Tilde{m}_j^{(i)}) + (1-\Tilde{m}_i^{(j)})  (1+\Tilde{m}_j^{(i)})} = \\
            &=     e^{2\beta_{aa'}} \frac{1+\Tilde{m}_i^{(j)}\Tilde{m}_j^{(i)}}{1-\Tilde{m}_i^{(j)}\Tilde{m}_j^{(i)}}  
        \label{expre_two_point}
        \end{align}
        valid for any boundary condition, and any depth $t$ of the tree $T_{ij}$. From now on we omit the $\Tilde{}$, calling the subtree magnetizations simply $m_a^{(a')}$ (doing so we lose nothing as the presence of the apex allows to distinguish them from the full system magnetizations). However, we know from the recursion that 
        $$m_i^{(j)}^{\boldsymbol{0}} \quad \xrightarrow[t\rightarrow \infty]{}  \quad  \bar{ m}_a^{(a')}^{\boldsymbol{0}} =  \tanh(\bar{z}_a^{(a')}^{\boldsymbol{0}})$$
        $$m_i^{(j)}^{\boldsymbol{+}} \quad \xrightarrow[t\rightarrow \infty]{}  \quad  \bar{m}_a^{(a')}^{\boldsymbol{+}} =  \tanh(\bar{z}_a^{(a')}^{\boldsymbol{+}})$$
        where $\bar{z}_a^{(a')}^{\boldsymbol{0}/\boldsymbol{+}}$ is the fixed point of the recursion with $\boldsymbol{0}/\boldsymbol{+}$ boundary conditions. We know that $\bar{z}_a^{(a')}^{\boldsymbol{0}} = \bar{z}_a^{(a')}^{\boldsymbol{+}} $ in the limit $t\rightarrow \infty$, so from now on we simply call $\bar{m}_a^{(a')}^{\boldsymbol{0}\boldsymbol{+}}= \bar{m}_a^{(a')}$. The same is also valid for $m_j^{(i)}^{\boldsymbol{0}/\boldsymbol{+}}$.
        Thus, applying the equalities in (\ref{expre_two_point}), taking the logarithm at both sides and inverting we get 
        \begin{align}
           <\sigma_i\sigma_j>_{T_{ij}(t)}^{\boldsymbol{0}/\boldsymbol{+}} \quad \xrightarrow[t\rightarrow \infty]{} & \quad \tanh \bigg( \beta_{aa'} + \tanh^{-1}(\bar{m}_{a'}^{(a')} \bar{m}_a'^{(a)})\bigg) \\
           & = \frac{\tanh(\beta_{aa'}) + \bar{m}_a^{(a')} \bar{m}_{a'}^{(a)} }{1+\tanh(\beta_{aa'}) \bar{m}_a^{(a')} \bar{m}_{a'}^{(a)} }
        \end{align}
        Moreover
        \begin{align}
            <\sigma_1 \sigma_2>_{G',\mu'} &=  \frac{e^{\beta_{aa'}+\bar{z}_a^{(a')}+\bar{z}_{a'}^{(a)}} + e^{\beta_{aa'}-\bar{z}_a^{(a')}-\bar{z}_{a'}^{(a)}} - e^{-\beta_{aa'}+\bar{z}_a^{(a')}-\bar{z}_{a'}^{(a)}} - e^{-\beta_{aa'}-\bar{z}_a^{(a')}+\bar{z}_{a'}^{(a)}} }{ e^{\beta_{aa'}+\bar{z}_a^{(a')}+\bar{z}_{a'}^{(a)}} + e^{\beta_{aa'}-\bar{z}_a^{(a')}-\bar{z}_{a'}^{(a)}} + e^{-\beta_{aa'}+\bar{z}_a^{(a')}-\bar{z}_{a'}^{(a)}} + e^{-\beta_{aa'}-\bar{z}_a^{(a')}+\bar{z}_{a'}^{(a)}} } \\
            &= \frac{\tanh(\beta_{aa'}) + \bar{m}_a^{(a')} \bar{m}_{a'}^{(a)} }{1+\tanh(\beta_{aa'}) \bar{m}_a^{(a')} \bar{m}_{a'}^{(a)} }
        \label{one_edge}
        \end{align}
        Thus (\ref{converg_eq}) is proved, and we have completed the second step of the theorem's proof.

        \vskip 0.8 cm

        \item The whole proof of this point consists of the computation of the derivative $\frac{\partial p(\boldsymbol{\beta},\boldsymbol{h})}{\partial \beta_{bb'}}$. Importantly, we will repeatedly use the fact that given a collection of variables $\{ x_i\}_{i=1}^n$ and real parameters $\{ \theta_j\}_{j=1}^n$, $h$  it holds $\forall \; i=1,...,n$ that 
        \begin{equation}
            \frac{e^h \prod_{j\neq i}^n (1+\theta_{j} x_j) - e^{-h} \prod_{j\neq i}^n (1-\theta_{j} x_j) }{e^h \prod_{j=1}^n (1+\theta_{j} x_j) + e^{-h} \prod_{j=1}^n (1-\theta_{j} x_j)} = \frac{G(x_1,...,x_{i-1},x_{i+1},...,x_n)}{1+\theta_{i} G(x_1,...,x_{i-1},x_{i+1},...,x_n)}
        \label{property_algebra}
        \end{equation}
        where 
        \begin{align}
            G(x_1,...,x_{i-1},x_{i+1},...,x_n) :&= \frac{e^h \prod_{j\neq i}^n (1+\theta_{j} x_j) - e^{-h} \prod_{j\neq i}^n (1-\theta_{j} x_j) }{e^h \prod_{j\neq i}^n (1+\theta_{j} x_j) + e^{-h} \prod_{j\neq i}^n (1-\theta_{j} x_j)} =\\
            &= \tanh\bigg(\log\bigg(e^h \prod_{j\neq i}^n \bigg(\frac{1+\theta_{j} x_j}{1-\theta_j x_j}\bigg)^\frac{1}{2}\bigg) \bigg) = \\
            &=  \tanh\bigg( h + \sum_{j\neq i} \tanh^{-1}(\theta_{j} x_j) \bigg)
        \label{G_x}
        \end{align}
        Thus, starting to compute 
        \begin{align}
            \frac{\partial p(\boldsymbol{\beta},\boldsymbol{h})}{\partial \beta_{bb'}} = \frac{\partial \theta_{bb'}}{\partial \beta_{bb'}} \frac{\partial p(\boldsymbol{\beta},\boldsymbol{h})}{\partial \theta_{bb'}} = (1-\theta_{bb'}^2) \frac{\partial p(\boldsymbol{\beta},\boldsymbol{h})}{\partial \theta_{bb'}} = (1-\theta_{bb'}^2) \frac{1}{2} \sum_{a=1}^n \alpha_a \frac{\partial F_a}{\partial \theta_{bb'}}
        \end{align}
        where 
        \begin{align}
            F_a &:= 2 \log\bigg( e^{h_a} \prod_{a'=1}^n \bigg(1+\theta_{aa'} \bar{m}_{a'}^{(a)}\bigg)^{k_{aa'}} - e^{-h_a} \prod_{a'=1}^n \bigg(1-\theta_{aa'} \bar{m}_{a'}^{(a)}\bigg)^{k_{aa'}} \bigg) +  \\
            &- \sum_{a'=1}^n k_{aa'} \bigg[ \frac{\log(1-\theta_{aa'}^2)}{2} + \log(\+\theta_{aa'} \bar{m}_{a}^{(a')} \bar{m}_{a'}^{(a)}) \bigg]
        \label{derivatives_freeen}
        \end{align}
        Paying attention that also each of the fixed points of the recursion $\bar{m}$ depends on each $\beta$ ($\theta$), and also that $\theta_{bb'}\equiv \theta_{b'b}$, we compute $\frac{\partial F_a}{\partial \theta_{bb'}}$ first for $b\neq b'$, in the cases of $a \neq b \;V\; a\neq b' $, $a=b$, $a=b'$:
        \begin{align}
            &\frac{\partial F_{a_{\neq b,b'}}}{\partial \theta_{bb'}} = \sum_{a'=1}^n C_{aa'} \\
            &\frac{\partial F_b}{\partial \theta_{bb'}} = k_{bb'}\bigg[ \frac{\theta_{bb'}}{1-\theta_{bb'}^2} + \frac{\bar{m}_b^{(b')}\bar{m}_{b'}^{(b)}}{g_{bb'}} \bigg]   +  \sum_{a'=1}^n C_{ba'} \\
            &\frac{\partial F_{b'}}{\partial \theta_{bb'}} = k_{b'b}\bigg[ \frac{\theta_{bb'}}{1-\theta_{bb'}^2} + \frac{\bar{m}_b^{(b')}\bar{m}_{b'}^{(b)}}{g_{bb'}} \bigg]   +  \sum_{a'=1}^n C_{b'a'} \\
        \end{align}
        where 
        \begin{align}
            &C_{\gamma\delta} := \frac{k_{\gamma\delta}\theta_{\gamma\delta}}{g_{\gamma\delta}} (\bar{m}_{\gamma}^{(\delta)} \frac{\partial \bar{m}_{\delta}^{(\gamma)}}{\partial \theta_{bb'}} -  \frac{\partial \bar{m}_{\gamma}^{(\delta)}}{\partial \theta_{bb'}} \bar{m}_{\delta}^{(\gamma)} ) \\
            & g_{\gamma\delta} := 1 + \theta_{\gamma\delta} \bar{m}_\gamma^{(\delta)}\bar{m}_{\delta}^{(\gamma)}
        \end{align}
        Notice that $ g_{\gamma\delta} =  g_{\delta\gamma}$.\\
        We have used property (\ref{property_algebra}) for computing the derivatives (\ref{derivatives_freeen}): for each $F_a$, we consider the vector $\boldsymbol{m_a} := (\bar{m}_1^{(a)}, ..., \bar{m}_1^{(a)}, \bar{m}_1^{(a)},...,\bar{m}_1^{(a)},  \;\;...\;\;, \bar{m}_n^{(a)},...,\bar{m}_n^{(a)})$ where each $\bar{m}_{a'}^{(a)}$ is repeated $k_{aa'}$ times, the parameters $\{\theta_{aa'}\}_{a'=1}^n$ and $h_a$; thus we apply equation (\ref{property_algebra}) noticing that defining  $G(\boldsymbol{m_a(i)})$, where $\boldsymbol{m_a(i)}$ is the same as $\boldsymbol{m_a}$ except for one missing entry of the type $\bar{m}_i^{(a)}$, it holds that (see eq. (\ref{G_x}) )
        $$G(\boldsymbol{m_a(i)}) =  \bar{m}_a^{(i)} $$
        At this point, in the case $b\neq b'$, we rewrite 
        \begin{align}
         \sum_{a=1}^n \alpha_a \frac{\partial F_a}{\partial \theta_{bb'}} &= \alpha_b \frac{\partial F_b}{\partial \theta_{bb'}} +\alpha_{b'}\frac{\partial F_{b'}}{\partial \theta_{bb'}}+ \sum_{a=1|a\neq b,b'}\alpha_a\frac{\partial F_a}{\partial \theta_{bb'}} =\\
         &= 2\alpha_bk_{bb'}\bigg[ \frac{\theta_{bb'}}{1-\theta_{bb'}^2} + \frac{\bar{m}_b^{(b')}\bar{m}_{b'}^{(b)}}{g_{bb'}} \bigg] + \alpha_b \sum_{a'=1}^n C_{ba'} + \alpha_{b'} \sum_{a'=1}^n C_{b'a'} + \sum_{a=1|a\neq b,b'}^n\alpha_a\sum_{a'=1}^n C_{aa'} =\\
         &= 2\alpha_bk_{bb'}\bigg[ \frac{\theta_{bb'}}{1-\theta_{bb'}^2} + \frac{\bar{m}_b^{(b')}\bar{m}_{b'}^{(b)}}{g_{bb'}} \bigg] + \sum_{a=1}^n\alpha_a\sum_{a'=1}^n C_{aa'} \\
         &= 2\alpha_bk_{bb'}\bigg[ \frac{\theta_{bb'}}{1-\theta_{bb'}^2} + \frac{\bar{m}_b^{(b')}\bar{m}_{b'}^{(b)}}{g_{bb'}} \bigg] 
        \end{align}
        where in the last step we used the fact that, since it holds $\forall \gamma,\delta = 1,...,n$ that $\alpha_\gamma C_{\gamma\delta} = \alpha_\delta C_{\delta\gamma}$ (as $\alpha_\gamma k_{\gamma\delta} = \alpha_\delta k_{\delta\gamma}$ by construction) and $C_{\gamma\gamma}=0 \; \forall \; \gamma=1,...,n$, then 
        $$\sum_{a=1}^n\alpha_a\sum_{a'=1}^n C_{aa'} = 0$$
        \\
        Now we deal with the case $b'=b$:
        \begin{align}
            &\frac{\partial F_{a_{\neq b}}}{\partial \theta_{bb}} = \sum_{a'=1}^n C_{aa'} \\
            &\frac{\partial F_b}{\partial \theta_{bb}} = k_{bb}\bigg[ \frac{\theta_{bb}}{1-\theta_{bb}^2} + \frac{\bar{m}_b^{(b)}^2}{g_{bb}} \bigg]   +  \sum_{a'\neq b}^n C_{ba'} 
        \end{align}
        by splitting the sum we get 
        \begin{align}
         \sum_{a=1}^n \alpha_a \frac{\partial F_a}{\partial \theta_{bb}} &= \alpha_b \frac{\partial F_b}{\partial \theta_{bb}} + \sum_{a\neq b}^n\alpha_a\frac{\partial F_a}{\partial \theta_{bb}} =\\
         &= \alpha_bk_{bb}\bigg[ \frac{\theta_{bb}}{1-\theta_{bb}^2} + \frac{\bar{m}_b^{(b)}^2}{g_{bb}} \bigg]   +  \alpha_b\sum_{a'\neq b}^n C_{ba'} +  \sum_{a\neq b}^n \alpha_a \sum_{a'=1}^n C_{aa'} \\
         &= \alpha_bk_{bb}\bigg[ \frac{\theta_{bb}}{1-\theta_{bb}^2} + \frac{\bar{m}_b^{(b)}^2}{g_{bb}} \bigg]   
        \end{align}
        for the same arguments as before.\\
        All in all, we get
        \begin{align}
            \frac{\partial p(\boldsymbol{\beta},\boldsymbol{h})}{\partial \beta_{bb'}} &=  (1-\theta_{bb'}^2) \frac{\alpha_bk_{bb'}}{2^{\delta_{bb'}}}\bigg[ \frac{\theta_{bb'}}{1-\theta_{bb'}^2} + \frac{\bar{m}_b^{(b')}\bar{m}_{b'}^{(b)}}{g_{bb'}} \bigg] =\\
            &=  \frac{\alpha_bk_{bb'}}{2^{\delta_{bb'}}}\bigg[ \frac{\theta_{bb'}+\bar{m}_b^{(b')}\bar{m}_{b'}^{(b)} }{1+\theta_{bb'}\bar{m}_b^{(b')}\bar{m}_{b'}^{(b)}}  \bigg]
        \end{align}
        and noticing again that 
        \begin{equation}
           \frac{\theta_{bb'}+\bar{m}_b^{(b')}\bar{m}_{b'}^{(b)} }{1+\theta_{bb'}\bar{m}_b^{(b')}\bar{m}_{b'}^{(b)}} = <\sigma_1 \sigma_2>_{G',\mu'}
        \end{equation}
        we have proved (\ref{derivative_functional}).
        
        \vskip 0.8 cm

        \item Now we know that $\mathbb{P}\bigg( \bigg|\frac{\partial p_N}{\partial \beta_{aa'}} - \frac{\partial p}{\partial \beta_{aa'}}\bigg|>\epsilon \bigg)  \xrightarrow[N\rightarrow \infty]{} 0 \quad \forall \;a,a'=1,...,n$, and $p_N(\boldsymbol{0},\boldsymbol{h})= p(\boldsymbol{0},\boldsymbol{h})$. Moreover, $\frac{\partial p_N}{\partial \beta_{aa'}}$ is uniformly bounded in $N$, as $\frac{\partial p_N}{\partial \beta_{aa'}} = \frac{1}{N} \sum_{<ij>\in E, i\in C_a, j\in C_{a'}} <\sigma_i \sigma_j>_{G_N} \leq \frac{|E_N|}{N} \leq C $ (the number of edges grows as $N$). Our aim is to prove that 
        \begin{equation}
            \mathbb{P}\bigg( |p_N(\boldsymbol{\beta},\boldsymbol{h}) -p(\boldsymbol{\beta},\boldsymbol{h})|>\epsilon \bigg)  \xrightarrow[N\rightarrow \infty]{} 0
        \label{final_pressure_covergence}
        \end{equation}       
        Thus, we first prove that 
        \begin{align}
            \lim_{N\rightarrow\infty} \mathbb{E} |p_N(\beta_{11},\boldsymbol{0},\boldsymbol{h}) &-p(\beta_{11},\boldsymbol{0},\boldsymbol{h})| = 0
        \label{first_l1_convergence}
        \end{align}
        For doing so, we exploit the fact that 
        \begin{align}
            \lim_{N\rightarrow\infty} \mathbb{E} \bigg|\frac{\partial p_N}{\partial \beta_{aa'}} - \frac{\partial p}{\partial \beta_{aa'}}\bigg| = 0
        \end{align}
        by Lebesgue's dominated convergence theorem, and so 
        \begin{align}
            \lim_{N\rightarrow\infty} \mathbb{E} \int_0^{\beta_{aa'}}\bigg|\frac{\partial p_N}{\partial \beta'_{aa'}} - \frac{\partial p}{\partial \beta'_{aa'}}\bigg| d\beta'_{aa'} = 0
        \end{align}
        for each $\beta_{aa'}$, by Fubini's theorem and again dominated convergence.\\
        Indeed 
        \begin{align}
            &\lim_{N\rightarrow\infty} \mathbb{E} |p_N(\beta_{11},\boldsymbol{0},\boldsymbol{h}) -p(\beta_{11},\boldsymbol{0},\boldsymbol{h})| = \\  
            &= \lim_{N\rightarrow\infty} \mathbb{E} |p_N(\boldsymbol{0},\boldsymbol{h}) -p(\boldsymbol{0},\boldsymbol{h}) + \int_0^{\beta_{11}}\bigg(\frac{\partial p_N}{\partial \beta'_{11}} - \frac{\partial p}{\partial \beta'_{11}}\bigg) d\beta'_{11}| = \\
            &= \lim_{N\rightarrow\infty} \mathbb{E} | \int_0^{\beta_{11}}\bigg|\frac{\partial p_N}{\partial \beta'_{11}} - \frac{\partial p}{\partial \beta'_{11}}\bigg| d\beta'_{11}| \leq\\
            &\leq \lim_{N\rightarrow\infty} \mathbb{E}  \int_0^{\beta_{11}}\bigg|\frac{\partial p_N}{\partial \beta'_{11}} - \frac{\partial p}{\partial \beta'_{11}}\bigg| d\beta'_{11} = 0\\          
        \end{align}
        Now exploiting (\ref{first_l1_convergence}) it is easy to prove that 
        \begin{align}
            \lim_{N\rightarrow\infty} \mathbb{E} |p_N(\beta_{11},\beta_{12},\boldsymbol{0},\boldsymbol{h}) &-p(\beta_{11},\beta{12},\boldsymbol{0},\boldsymbol{h})| = 0
        \end{align}
        indeed 
        \begin{align}
            &\lim_{N\rightarrow\infty} \mathbb{E} |p_N(\beta_{11},\beta_{12},\boldsymbol{0},\boldsymbol{h}) -p(\beta_{11},\beta{12},\boldsymbol{0},\boldsymbol{h})| \leq \\
            &\leq \lim_{N\rightarrow\infty} \mathbb{E} |p_N(\beta_{11},\boldsymbol{0},\boldsymbol{h}) -p(\beta_{11},\boldsymbol{0},\boldsymbol{h})| + \mathbb{E}\int_0^{\beta_{12}}\bigg|\frac{\partial p_N}{\partial \beta'_{12}} - \frac{\partial p}{\partial \beta'_{12}}\bigg| d\beta'_{12} = 0 \\            
        \end{align}
        And so, iterating the process for all until $\beta_{nn}$, we eventually get
        \begin{align}
            \lim_{N\rightarrow\infty} \mathbb{E} |p_N(\boldsymbol{\beta},\boldsymbol{h}) &-p(\boldsymbol{\beta},\boldsymbol{h})| = 0
        \end{align}  
        from which (\ref{final_pressure_covergence}) follows as $L^1$ convergence implies convergence in probability.
        




        
        % Thus we write 
        % \begin{align}
        %     |p_N(\boldsymbol{\beta},\boldsymbol{h}) &-p(\boldsymbol{\beta},\boldsymbol{h})| =\\
        %     &=|p_N(t\boldsymbol{\beta},\boldsymbol{h})\bigg|_{t=1}-p(t\boldsymbol{\beta},\boldsymbol{h})\bigg|_{t=1}| = \\
        %     &= |\; p_N(\boldsymbol{0},\boldsymbol{h}) + \int_{0}^{1} \frac{\partial p_N(t'\boldsymbol{\beta},\boldsymbol{h})}{\partial {t'}} dt'  - p(\boldsymbol{0},\boldsymbol{h}) - \int_{0}^{1} \frac{\partial p(t'\boldsymbol{\beta},\boldsymbol{h})}{\partial {t'}} dt' \;| = \\
        %     &= |\;  \int_{0}^{1} \bigg(\frac{\partial p_N(t'\boldsymbol{\beta},\boldsymbol{h})}{\partial {t'}} - \frac{\partial p(t'\boldsymbol{\beta},\boldsymbol{h})}{\partial {t'}} \bigg) dt'  \;| = \\
        %     &= |\;  \int_{0}^{1} \bigg( <\boldsymbol{\nabla} p_N(t'\boldsymbol{\beta},\boldsymbol{h}), \boldsymbol{\beta}> -  <\boldsymbol{\nabla} p(t'\boldsymbol{\beta},\boldsymbol{h}), \boldsymbol{\beta}> \bigg) dt'  \;| = \\
        %     &= |\; \sum_{a,a'=1,...,n} \beta'_{aa'}\int_{0}^{1} \bigg(\frac{\partial p_N(\boldsymbol{\beta'},\boldsymbol{h})}{\partial {\beta'_{aa'}}} - \frac{\partial p_N(\boldsymbol{\beta'},\boldsymbol{h})}{\partial {\beta'_{aa'}}} \bigg) dt'  \;|
        % \end{align}
        % where $\beta'_{aa'} := t'\beta_{aa'}$. We have used the fundamental theorem of calculus, the chain rule and the result of point 1. Now as for points 2 and 3 all the integrands converge in probability and are bounded, then (\ref{final_pressure_covergence}) follows by dominated convergence (DISCUTERNE).

    {\color{red}OLD PROOF of point 3 DELETED FROM MAIN (changed by Diego): We compute 
        \begin{equation}
            \frac{\partial f_a}{\partial \theta_{bb'}} =  \sum_{a'\in \mathcal E_a} \bigg[ C_{aa'} + k_{aa'}\bigg( \frac{\theta_{aa'}}{1-\theta_{aa'}^2} + \frac{\bar{m}_a^{(a')}\bar{m}_{a'}^{(a)}}{g_{aa'}} \bigg) \frac{(\delta_{ab}\delta_{a'b'} + \delta_{ab'}\delta_{a'b})}{2^{\delta_{bb'}}}\bigg]
        \label{derivative_3point_pressure}
        \end{equation}
        where 
        \begin{align}
            &C_{cd} \,:=\, \frac{k_{cd}\,\theta_{cd}}{g_{cd}} \bigg(\bar{m}_{c}^{(d)}\, \frac{\partial \bar{m}_{d}^{(c)}}{\partial \theta_{bb'}} -  \frac{\partial \bar{m}_{c}^{(d)}}{\partial \theta_{bb'}}\,\bar{m}_{d}^{(c)} \bigg) \\
            & g_{cd} \,:=\, 1 + \theta_{cd}\, \bar{m}_c^{(d)}\bar{m}_{d}^{(c)} \,=\,  g_{dc}
        \end{align}
        We have used property (\ref{property_algebra}) to compute \eqref{derivative_3point_pressure}: given $a\leq n$, we consider the vector
        \begin{equation}
        \boldsymbol{x}^{(a)} :=\, \big(\underbrace{\theta_{a1}\,\bar{m}_1^{(a)}, \dots, \theta_{a1}\,\bar{m}_1^{(a)}}_{k_{a1}\textrm{ times}},\, \underbrace{\theta_{a2}\,\bar{m}_2^{(a)},\dots,\theta_{a2}\,\bar{m}_2^{(a)}}_{k_{a2}\textrm{ times}},\, \dots\dots,\, \underbrace{\theta_{an}\,\bar{m}_n^{(a)},\dots,\theta_{an}\,\bar{m}_n^{(a)}}_{k_{an}\textrm{ times}}\big)
        \end{equation}
        where each element $\theta_{aa'}\,\bar{m}_{a'}^{(a)}$ is repeated $k_{aa'}$ times.  
        Then for every $a'\in\mathcal E_a$, define the vector $\boldsymbol{x}^{(a)}_{-a'}$ by removing from $\boldsymbol{x}^{(a)}$ only one component of the type $\theta_{aa'}\,\bar{m}_{a'}^{(a)}$.
        Thus we apply equation (\ref{property_algebra}) noticing that , it holds that (see eq. (\ref{G_x}) )
        $$G(\boldsymbol{\bar{m}^{(a)}_{-a'}}) =  \bar{m}_a^{(a')} $$
        Then we can write 
        \begin{equation}
        \begin{split}
         \sum_{a=1}^n \alpha_a \frac{\partial f_a}{\partial \theta_{bb'}} 
         &= \frac{2\alpha_bk_{bb'}}{2^{\delta_{bb'}}}\bigg[ \frac{\theta_{bb'}}{1-\theta_{bb'}^2} + \frac{\bar{m}_b^{(b')}\bar{m}_{b'}^{(b)}}{g_{bb'}} \bigg] + \sum_{a=1}^n\alpha_a\sum_{a'\in \mathcal E_a} C_{aa'} \\
         &= \frac{2\alpha_bk_{bb'}}{2^{\delta_{bb'}}}\bigg[ \frac{\theta_{bb'}}{1-\theta_{bb'}^2} + \frac{\bar{m}_b^{(b')}\bar{m}_{b'}^{(b)}}{g_{bb'}} \bigg] 
        \end{split}
        \end{equation}
        where we have used the fact that, since it holds $\forall c,d = 1,...,n$ that $\alpha_c C_{cd} = \alpha_d C_{cd}$ (as $\alpha_c k_{cd} = \alpha_d k_{dc}$ by construction), $C_{cc}=0 \; \forall \; c=1,...,n$, and if $(a,b)\in \mathcal E$ then also $(b,a)\in \mathcal E$, then 
        \begin{equation}
            \sum_{a=1}^n\alpha_a\sum_{a' \in \mathcal E_a} C_{aa'} = 0
        \end{equation}
        
        Eventually, we get
        \begin{equation}
        \begin{split}
            \frac{\partial p(\boldsymbol{\beta},\boldsymbol{h})}{\partial \beta_{bb'}} &=  (1-\theta_{bb'}^2) \frac{\alpha_bk_{bb'}}{2^{\delta_{bb'}}}\bigg[ \frac{\theta_{bb'}}{1-\theta_{bb'}^2} + \frac{\bar{m}_b^{(b')}\bar{m}_{b'}^{(b)}}{g_{bb'}} \bigg] \\
            &=  \frac{\alpha_bk_{bb'}}{2^{\delta_{bb'}}}\bigg[ \frac{\theta_{bb'}+\bar{m}_b^{(b')}\bar{m}_{b'}^{(b)} }{1+\theta_{bb'}\bar{m}_b^{(b')}\bar{m}_{b'}^{(b)}}  \bigg]
        \end{split}
        \end{equation}
        and noticing again that 
        \begin{equation}
           \frac{\theta_{bb'}+\bar{m}_b^{(b')}\bar{m}_{b'}^{(b)} }{1+\theta_{bb'}\,\bar{m}_b^{(b')}\bar{m}_{b'}^{(b)}} \,=\, \langle\sigma_1 \sigma_2\rangle_{aa'}
        \end{equation}
        we have proved (\ref{derivative_functional}).}
        
    \end{enumerate}
    

    
    
    



    
\end{proof}


\begin{remark}
    The quantity $p(\boldsymbol{\beta},\boldsymbol{h})$ is referred as pressure or free entropy per paticle in literature. The free energy density is simply equal to $-p_N(\boldsymbol{\beta},\boldsymbol{h})$. Notice that the function $-p(\boldsymbol{\beta},\boldsymbol{h})$ corresponds to the Bethe free energy density (see e.g. \cite{dembo2010gibbs}, Proposition 3.9) calculated at the cavity fields of the BP algorithm (or Bethe recursion) equal to the fixed point of our recursion $\boldsymbol{\bar{z}}$.
\end{remark}

\begin{remark}
        One can easily verify that
        \begin{equation}
            \frac{\partial p_N(\boldsymbol{\beta},\boldsymbol{h})}{\partial h_a} = \frac{1}{N} \sum_{i\in C_a} <\sigma_i> \;\xrightarrow[N\rightarrow \infty]{\Pprob}\; \frac{\partial p(\boldsymbol{\beta},\boldsymbol{h})}{\partial h_a}
        \end{equation}
\end{remark}

==> From_trees_to_graphs/pos_field.tex <==
\begin{theorem}
    Consider a random $\mathbf{k}$-regular graph $G_N$ with $n$ classes $C_1,...,C_n$. Consider an Ising model on $G_N$ with all non-negative external fields associated to the classes $h_i$, $i= 1,...,n$, and ferromagnetic (positive) couplings $\beta_{ij}$ depending only on the classes of the interacting spins. For every class $C_i$, the equilibrium magnetization of each spin $x\in C_i$ in $G_N$, for large $N$, converges in probability to
    $$<\sigma_x>_{G_N} \quad \xrightarrow[N\rightarrow\infty]{\Pprob} \quad  \tanh\bigg( h_i + \sum_{k} k_{ik} F_{\beta_{ik}}(\bar{z}_k^{(i)}) \bigg)$$
    where $F_\beta(y) = \tanh^{-1}\bigg( \tanh(\beta) \tanh(y)\bigg)$ and $\{\bar{z}_i^{(j)}\}_{i,j=1,...,n}$ is the unique fixed point of the $n^2$-dimensional recursion
    $$z_i^{(j)} (s) = h_i + \sum_{k} (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(z_k^{(i)} (s-1)) \;\;\;\;\;\; \forall\;i,j = 1,...,n$$
    reached for any non-negative initialization.
\label{th_positive_fields_magnetization}
\end{theorem}

\begin{proof}
   Indicate as $<\sigma_x>_{G_N}$ the average under the Ising measure, i.e. the equilibrium magnetization, of a spin at site $x$ in $G_N$ belonging to class $C_i$ ($x\in I_i$). 
   % By simmetry, all the spins in $C_i$ will have the same magnetization, that we indicate indeed with $<\sigma_i>_{G_N}$. 
   Consider a ball in $G_N$ centered in node $x$ of radius $t$, $B(x,t)$. 
   Then, consider the Ising model on the subgraph corresponding to the ball, with free and positive boundary conditions (corresponding to no added fields and infinite fields to the node at the boundary). We indicate by $<\sigma_x>^0_{B(x,t)}$ and $<\sigma_x>^+_{B(x,t)}$ the equilibrium magnetization of spin $x$ respectively under free and plus boundary conditions. By GKS inequalities, applying the same considerations as in the trees before (addition of edges and removal of fields), we find that 
   $$<\sigma_x>^0_{B(x,t)} \;\;\leq \;\; <\sigma_x>_{G_N} \;\;\leq \;\; <\sigma_x>^+_{B(x,t)}$$    
   Now indicate with $T(x,t)$ a random $\mathbf{k}$-regular tree with the same classes and degrees of $G_N$, depth $t$, rooted in node $x$, which belongs to class $C_i$. From Theorem \ref{th: tree-like} we have that with probability $1$ for $N\rightarrow \infty$ the subgraph coinciding with the ball $B(x,t)$ and $T(\mathbf{k},x,t)$ are isomorphic. Then, indicating with $<\sigma_x>^{0/+}_{T(x,t)}$ the averages under the Ising measure on the tree, 
   % $$<\sigma_x>^0_{T(x,t)} \;\;\leq \;\;\lim_{N\rightarrow \infty}<\sigma_x>_{G_N} \;\;\leq \;\; <\sigma_x>^+_{T(x,t)}$$  
   from Corollary \ref{} we have that both 
   $$<\sigma_x>^+_{T(x,t)} \Searrow \; m^*_x \;\;\;\;\;\;\;  <\sigma_i>^0_{T(x,t)} \Nearrow \; m^*_x  \;\;\;\;\;\;\; \mbox{for}\;t\rightarrow \infty$$
   where 
   $$m^*_x = \tanh\bigg( h_i + \sum_{k} k_{ik} F_{\beta_{ik}}(\bar{z}_k^{(i)}) \bigg)$$
   with $F_\beta(y) = \tanh^{-1}\bigg( \tanh(\beta) \tanh(y)\bigg)$ and $\{\bar{z}_i^{(j)}\}_{i,j=1,...,n}$ is the unique fixed point of the $n^2$-dimensional recursion
   $$z_i^{(j)} (s) = h_i + \sum_{k} (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(z_k^{(i)} (s-1)) \;\;\;\;\;\; \forall\;i,j = 1,...,n$$
   reached for any non-negative initialization.\\
   \\
   We can write 
   \begin{align}
       <\sigma_x>_{G_N} -\; m^*_x \;\; &\leq \;\; <\sigma_x>^+_{B(x,t)} - \; m^*_x =\\
       &=\; <\sigma_x>^+_{B(x,t)}-<\sigma_x>^+_{T(x,t)} + <\sigma_x>^+_{T(x,t)}  - \; m^*_x
   \end{align}
   where, fixing $\epsilon>0,\; \delta>0$, 
   $$ <\sigma_x>^+_{T(x,t)}  - \; m^*_x  <\epsilon  \quad \forall \; t>t_\epsilon$$
   $$\Pprob\bigg(<\sigma_x>^+_{B(x,t)}-<\sigma_x>^+_{T(x,t)} \neq 0 \bigg) <\delta  \quad \forall \; N>N_{\delta,t_\epsilon}$$
   respectively for the monotonicity and uniqueness arguments of the previous paragraphs and the isomorphism between the ball and the truncated tree. Same thing for the lower bound
   \begin{align}
       m^*_x - <\sigma_x>_{G_N}  \;\; &\leq \;\; m^*_x - <\sigma_x>^0_{B(x,t)}  =\\
       &= m^*_x - <\sigma_x>^0_{T(x,t)} + <\sigma_x>^0_{T(x,t)}- <\sigma_x>^0_{B(x,t)}
   \end{align}
   where, fixing $\epsilon>0,\; \delta>0$, 
   $$ m^*_x - <\sigma_x>^0_{T(x,t)}  <\epsilon  \quad \forall \; t>t_\epsilon$$
   $$\Pprob\bigg(<\sigma_x>^0_{B(x,t)}-<\sigma_x>^0_{T(x,t)} \neq 0 \bigg) <\delta  \quad \forall \; N>N_{\delta,t_\epsilon}$$
   Therefore for any $\epsilon>0,\; \delta>0$, and $t_\epsilon$ accordingly 
   $$\Pprob\bigg(| <\sigma_x>_{G_N} -\; m^*_x| \geq \epsilon \bigg)< 2\delta  \quad \forall \; N>N_{\delta,t_\epsilon}$$
   that is 
   $$<\sigma_x>_{G_N} \quad \xrightarrow[N\rightarrow \infty]{\Pprob} \quad  m^*_x$$
   in probability, for any spin $x \in I_i \;\; \mbox{(class}\; C_i)$.\\  
   % As the two bounds approach to the same limit, $\lim_{N\rightarrow \infty}<\sigma_x>_{G_N} = m_i$ almost surely. Importantly, note that once specified the class of the root and the depth, the realization of the tree $T(\mathbf{k},x,t)$ is unique, and so are the bounds: thus,
   % $$\lim_{N\rightarrow \infty}<\sigma_x>_{G_N} = \lim_{N\rightarrow \infty}<\sigma_y>_{G_N}\;\;\;\;\; \forall\; x,y\in I_i \;\; \mbox{(class}\; C_i)$$  
   The same procedure is applied taking as root of the ball (and the tree) a node of each of the $n$ classes.  
\end{proof}

==> From_trees_to_graphs/tree_like.tex <==
\begin{theorem}
    Fix $t<\infty$ and a positive integer $I$. The probability $Q(N,t)$ that the closed ball of radius $t$ and center $I$ in a random $\mathbf{k}-$regular graph $G_N$ converges to one as $N\rightarrow\infty$.
\label{th: tree-like}
\end{theorem}

\begin{proof}
    Let $B_N(t)$ denote the subgraph of radius $t$ and center $i$ in $G$. Depending on the distance from the root,
    $$1- Q(N,t) \sim N^{-1}$$
    indeed 
    $$Q(N,t) = \prod_{j=0}^{\gamma(i,k_{kl},t)} (1-q(v))$$
    where $\gamma(t)$ represents the number of nodes within the radius $t$ and is a function of the chosen center and the degrees. $q(v)$ instead is the probability that the $v-$th generated node has a link shared with previously generated nodes, i.e. that $B(t)$ is not a tree. It is easy to see that 
    $$q(v) = C(v,i,\mathbf{k},t)/N$$
    where $C$ does not depend on $N$. Thus 
    $$Q(N,t) = 1 - \frac{C_{max}}{N} + O(N^{-2})$$
\end{proof}

==> Preliminaries/inequalities.tex <==
We consider an Ising spin system of $N$ binary spins, $\sigma_i=\{-1,+1\}$ for $i= 1,...,N$, on a general graph $G_N(V,E)$, $|V|=N$, with Hamiltonian 
\begin{equation}
    H(\boldsymbol{\sigma}) = \sum_{(i,j)\in E}\beta_{ij}\sigma_i\sigma_j + \sum_{i\in V}h_i\sigma_i
\label{general hamiltonian}
\end{equation}
Under the Gibbs (Boltzmann) measure 
$$\mu_I (\boldsymbol{\sigma}) = \frac{e^{H(\boldsymbol{\sigma})}}{\sum_{\boldsymbol{\sigma}} e^{H(\boldsymbol{\sigma})}} $$
so expressing the average of an observable (function of the spins) as
$$<f(\boldsymbol{\sigma})> = \sum_{\boldsymbol{\sigma}}\frac{f(\boldsymbol{\sigma}) e^{H(\boldsymbol{\sigma})}}{\sum_{\boldsymbol{\sigma}} e^{H(\boldsymbol{\sigma})}}$$
the following inequalities, under the corresponding assumptions on the Hamiltonian, hold. Before listing the inequalities, let us also recall that defining $m_i = <\sigma_i>$ we have that
$\frac{\partial \;m_i}{\partial\;h_j} =$\small$ <\sigma_i \sigma_j> -  <\sigma_i>< \sigma_j>$ and\\
$\frac{\partial^2 \;m_i}{\partial\;h_j\;\partial\;h_k} = $\small$<\sigma_i \sigma_j \sigma_k> + 2<\sigma_i>< \sigma_j>< \sigma_k> - (<\sigma_i>< \sigma_j \sigma_k> + <\sigma_j>< \sigma_i \sigma_k> + <\sigma_k>< \sigma_i \sigma_j> )$.
\vskip 1cm
\begin{theorem}[GKS inequalities]
    If $h_i\geq0 \;\forall \;i$, $\;\;\beta_{ij}\geq0 \;\forall\;i,j\;\;$    then
    $$<\sigma_A \sigma_B> \;\geq\; <\sigma_A>< \sigma_B>$$
    where $A,B\subseteq V$ and $\sigma_{A/B} = \prod_{i\in A/B} \sigma_i$.
\end{theorem}
\begin{remark}
    Under the conditions of the GKS, $\forall i,j,k$
    $$\frac{\partial \;m_i}{\partial\;h_j} = <\sigma_i \sigma_j> -  <\sigma_i>< \sigma_j> \;\geq 0$$
    $$\frac{\partial \;m_i}{\partial\;\beta_{jk}} = <\sigma_i \sigma_j \sigma_k> -  <\sigma_i>< \sigma_j\sigma_k> \;\geq 0$$
\end{remark}
\vskip 1cm
\begin{theorem}[FKG inequalities]
    For any vector of fields $\mathbf{h}$, for $\beta_{ij}\geq0 \;\forall\;i,j\;\;$, if $f(\vec{\sigma})$ and $g(\vec{\sigma})$ are increasing functions of the spins, in the sense that $f(\vec{\sigma}) \equiv f(\sigma_1,...\sigma_i,...,\sigma_N)$  is such that
    $$f(\sigma_1,...\sigma_i=-1,...,\sigma_N) \leq f(\sigma_1,...\sigma_i=1,...,\sigma_N)$$
    for any $i$, and same for $g(\vec{\sigma})$; then 
    $$<fg>\;\geq\;<f><g>$$
\end{theorem}
\begin{remark}
    If $\beta_{ij}\geq0, \;\forall\;i,j\;\;$
    $$\frac{\partial \;m_i}{\partial\;h_j} = <\sigma_i \sigma_j> -  <\sigma_i>< \sigma_j> \;\geq 0$$
    (since we apply FKG inequality choosing $f(\vec{\sigma}) = \sigma_i$ and $g(\vec{\sigma}) = \sigma_j$, both increasing functions).
\end{remark}
\vskip 1cm
\begin{theorem}[GHS inequalities]
    If $h_i\geq0 \;\forall \;i$, $\;\;\beta_{ij}\geq0 \;\forall\;i,j\;\;$    then
    $$\frac{\partial^2 \;m_i}{\partial\;h_j\;\partial\;h_k}\leq 0$$
    $\forall \; i,j,k$ not necesairly distinct.
\end{theorem}
% \begin{remark}
%     Under the assumptions of the GHS, the magneization at any site $i$ is concave with respect to the external magnetic field at any site $j$, as 
%     $$\frac{\partial^2 \;m_i}{\partial\;h_j ^2} \leq 0 $$
% \end{remark}


==> Preliminaries/recursion.tex <==
In the following we consider the Gibbs measure with Hamiltonian (\ref{general hamiltonian}) for $G=T$ general tree, that we indicate with $\mu_T(\sigma)$. 

\begin{lemma}
    Let $T$ be a tree, $v$ one of its vertex that we call the root, and $w$ a vertex at distance $d_v(w)$ from the root (if $d_v(w)=0$ then $w\equiv v$). Indicate with $T_w$ the subtree of $T$ having as vertices $w$ (its root) and all its connected vertices at distances greater than $d_v(w)$ from the root $v$ of $T$. Let $\{u_1,...,u_K\}$ be the vertices of $T_w$ that are adjacent to $w$ in $T_w$, $K_w$ the degree of $w$ in $T_w$. For $u_i=1,...,K(w)$ let $T_{u_i}$ denote the sub-tree of $T_w$ with root $u_i$ after the removal of the edge $(w,u_i)$. Indicating with $\Tilde{m}_j = \mu_{T_j}(\sigma_j=1) - \mu_{T_j}(x_\sigma=-1)$ the magnetization of a node $j$ for the Ising measure restricted to the associated subtree $T_j$ (with root $j$), and taking $z_j := \tanh^{-1}(\Tilde{m}_j)$, we have that 
    \begin{equation}
        z_w = h_w + \sum_{i=1}^{K_w} F_{\beta_{wu_i}}(z_{u_i})
    \label{lemma1}
    \end{equation}   
    where 
    \begin{equation}
        F_\beta(y) := \tanh^{-1}(\tanh(\beta)\tanh(y))
    \label{F_beta definition}
    \end{equation}
    \\
\label{recursion_generic_tree}
\end{lemma}
\begin{remark}
    When initiated with the root $v$ of the tree, then $T_v\equiv T$ and the recursion leads to the root magnetization $m_v\equiv \Tilde{m_v}=\mu_T(\sigma_v=1) - \mu_T(\sigma_v=-1)$. 
\end{remark}
\begin{remark}
    If $u\in T_*$, meaning that the node $u$ belongs to the boundary of the tree $T$, then the associated subgraph $T_u$ consists solely in the node itself and thus 
    $$z_u = h_u$$
    which is indeed the initialization of the recursion. 
\end{remark}


\begin{proof}
    Let $H_{T_w}(\boldsymbol{\sigma}_{T_w}) = \sum_{(i,j)\in T_w} \beta_{ij} \sigma_i\sigma_j + \sum_{i\in T_w} h_i \sigma_i $ be the contribution to $H(\boldsymbol{\sigma})$ (\ref{general hamiltonian}) from the vertices and edges within $T_w$. Denoting with $T_{u_i}$ the smaller subtrees having as roots the neighbours of $w$ in $T_w$, namely $u_i = 1,...,K_w$ ($K_w$ is the degree of $w$ in $T_w$), we can write $H_{T_w}(\boldsymbol{\sigma}_{T_w})$ in terms of the contribution of such smaller subtrees 
    $$H_{T_w}(\boldsymbol{\sigma}_{T_w}) = \sum_{i=1}^{K_w} H_{T_{u_i}}(\boldsymbol{\sigma}_{T_{u_i}})   +  h_w\sigma_w + \sigma_w  \sum_{i=1}^{K_w} \beta_{wu_i}\sigma_{u_i} $$
    Defining $S_{w;T_w}(\xi) = \mu_{T_w}(\sigma_w=\xi)$ for $\xi\in\{+1,-1\}$
    \begin{align}
     S_{w;T_w}(\xi) &= \frac{1}{Z_{T_w}} \sum_{\boldsymbol{\sigma}_{T_w}:\sigma_w=\xi} e^{H_{T_w}(\boldsymbol{\sigma}_{T_w})}  \\
     &= \frac{e^{\xi h_w}}{Z_{T_w}} \prod_{i=1}^{K_w} \;\sum_{\boldsymbol{\sigma}_{T_{u_i}}} e^{\beta_{wu_i} \xi \sigma_{u_i}} \;\;e^{H_{T_{u_i}}(\boldsymbol{\sigma}_{T_{u_i}})}  \\
     &= \frac{e^{\xi h_w}}{Z_{T_w}} \prod_{i=1}^{K_w} \;\bigg[  e^{\beta_{wu_i} \xi} \sum_{\boldsymbol{\sigma}_{T_{u_i}}: \sigma_{u_i}=1} e^{H_{T_{u_i}}(\boldsymbol{\sigma}_{T_{u_i}})}  +  e^{-\beta_{wu_i} \xi} \sum_{\boldsymbol{\sigma}_{T_{u_i}}: \sigma_{u_i}=-1} e^{H_{T_{u_i}}(\boldsymbol{\sigma}_{T_{u_i}})} \bigg]\\
     &= \frac{e^{\xi h_w}}{Z_{T_w}} \prod_{i=1}^{K_w} \;Z_{T_{u_i}}   \bigg[ e^{\beta_{wu_i} \xi} S_{u_i; T_{u_i}}(+1) + e^{-\beta_{wu_i} \xi} S_{u_i; T_{u_i}}(-1) \bigg] \\
     &= \frac{\prod_{i=1}^{K_w}Z_{T_{u_i}}} {Z_{T_w}} e^{\xi h_w} \prod_{i=1}^{K_w} \;  \bigg[ e^{\beta_{wu_i} \xi} S_{u_i; T_{u_i}}(+1) + e^{-\beta_{wu_i} \xi} S_{u_i; T_{u_i}}(-1) \bigg] \\
    \end{align}
    from which 
    $$  \frac{S_{w;T_w}(+1)}{S_{w;T_w}(-1)}  = \frac{e^{ h_w} \prod_{i=1}^{K_w} \;  \bigg[ e^{\beta_{wu_i}} S_{u_i; T_{u_i}}(+1) + e^{-\beta_{wu_i}} S_{u_i; T_{u_i}}(-1) \bigg]}{ e^{-h_w} \prod_{i=1}^{K_w} \;  \bigg[ e^{-\beta_{wu_i} } S_{u_i; T_{u_i}}(+1) + e^{\beta_{wu_i}} S_{u_i; T_{u_i}}(-1) \bigg] } $$
    Noticing that $S_{w;T_w}(\xi) = \frac{1+\xi\Tilde{m}_w}{2}$ and $\frac{S_{w;T_w}(+1)}{S_{w;T_w}(-1)} = \frac{1+\Tilde{m}_w}{1-\Tilde{m}_w}$ 
    $$ \frac{1+\Tilde{m}_w}{1-\Tilde{m}_w} = \frac{e^{ h_w} \prod_{i=1}^{K_w} \bigg[ e^{\beta_{wu_i}} (1+\Tilde{m}_{u_i}) + e^{-\beta_{wu_i}} (1-\Tilde{m}_{u_i}) \bigg] }{e^{-h_w} \prod_{i=1}^{K_w} \bigg[ e^{-\beta_{wu_i}} (1+\Tilde{m}_{u_i}) + e^{\beta_{wu_i}} (1-\Tilde{m}_{u_i}) \bigg]}  $$
    applying half the logarithm at both sides we get
    $$\tanh^{-1}(\Tilde{m}_w) = h_w + \sum_{i=1}^{K_w} \tanh^{-1}(\tanh(\beta_{wu_i})\Tilde{m}_{u_i}) $$
    which is exactly (\ref{lemma1}), upon verifying that 
    $$  \frac{e^{\beta} (1+x) + e^{-\beta} (1-x)}{e^{-\beta} (1+x) + e^{\beta} (1-x)} =  \tanh^{-1}(\tanh(\beta)x) $$
\end{proof}
 
\vskip 2 cm

\begin{definition}
    Consider $1,...,n$ classes and a matrix of degrees $\mathbf{k}$. A $\mathbf{k}$-regular tree rooted in $v\in C_v$ of depth $t$, namely $T_v(\mathbf{k},t)$, is constructed as follows: starting from the root, create the first generation of $k_{vj}$ nodes for each class $j$ and connect each node to the root; recursively, from each node of class $C_i$ $i=1,...,n$ of the $d-th$ generation with connection to a node of class $C_j$ of the previous generation originate $k_{ij}-1$ "children" of class $C_j$ and $k_{ig}$ of class $C_g$, for $g=1,...,j-1,j+1,..,n$; we indicate a node of this type as $(i(j), d)$, and the subtree rooted in $(i(j), d)$ which includes all the vertices of successive generations as $T_{i(j)}(\mathbf{k},d)$. The recursive construction stops at the $t-$th generation.  
\end{definition}

\begin{remark}
    Contrairly to random $\mathbf{k}$-regular graph, the realization of a $\mathbf{k}$-regular tree, given the root's class and the depth, is unique. Also the realization of any of the subtrees $T_{i(j)}(\mathbf{k},d)$ is unique. ("the tree is fully characterized by $(i(j),d)$") 
\end{remark}

\vskip 1 cm

\begin{corollary}
    Consider a $\mathbf{k}$-regular tree rooted in $v\in C_v$ of depth $t$, $T_v(\mathbf{k},t)$. To each spin of one class, e.g. $C_i$, is associated the same magnetic field $h_i$; moreover, the couplings depend only on the classes of the extremes $C_i,C_j$ and $\beta_{ij}= \beta_{ji}$. With the exception of the root, for each node of type $(i(j),d)$ we indicate with $\Tilde{m}^{(j)}_i(d) = \mu_{T_{i(j)}(\mathbf{k},d)}(\sigma_j=1) - \mu_{T_{i(j)}(\mathbf{k},d)}(\sigma_j=-1)$ its magnetization for the Ising measure restricted to the associated subtree $T_{i(j)}(\mathbf{k},d)$, and take $z^{(j)}_i(d) = \tanh^{-1}(\Tilde{m}^{(j)}_i(d))$. 
    % Indicating with $s=t-d$ the distance from the boundary of $T_v(\mathbf{k},t)$, instead of considering $z^{(j)}_i(d)$ we consider $z^{(j)}_i(s=t-d)$. The following recursion holds for $s=1,...,t-1$ HO LASCIATO RICORSIONE AL CONTRARIO
    The following recursion holds for $d=t-1,...,1$
    \begin{equation}
        z_i^{(j)} (d) = h_i + \sum_{g} (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(z_k^{(i)} (d+1)) \;\;\;\;\;\; \forall\;i,j = 1,...,n
    \label{recursion_regular_trees}
    \end{equation}   
    initialized ($d=t$) by
    \begin{equation}
        z_i^{(j)} (t) = h_i  \;\;\;\;\;\; \forall\;i,j = 1,...,n
    \label{initialization_recursion_regular_trees}
    \end{equation}
    where $F_\beta(x)$ is defined in (\ref{F_beta definition}) and $\delta_{jk}$ is the Kronecker delta. \\
    For the magnetization at the root $z_v = \tanh^{-1}(m_v)$ we have
    $$z_v = h_v + \sum_{k} k_{ik} F_{\beta_{ik}}(z_k^{(i)} (1)) $$   
\end{corollary} 

\begin{proof}
    Since the realizations of the corresponding subtree (and the boundary conditions) are isomorphic for any nodes of the same type $(i(j),d)$, then also the corresponding subtree magnetizations $z^{(j)}_i(d)$ must be the same. Once considered this, the corollary comes straight from the application of the recursive relations in Lemma \ref{recursion_generic_tree}.     
\end{proof}
Note that with a little abuse of notation we have used at the same time $k_{ij}$ for the degrees and little $k$ for the indices of the classes. 


==> old_versions.tex <==
% \\
% * in questo caso si vede che la matrice è primitiva vedendo che $(M^2)_{ij}>0$: ponendo $1$ su tutti i valori di $M$ diversi da zero, si vede ordinando le entrate $(1,1),(1,2),...,(n,n)$ che dividendo i vettori riga e colonna in gruppi da $n$, i vettori riga avranno esattamente un $1$ in ogni gruppo, mentre i vettori colonna hanno $n-1$ gruppi di tutti zeri e uno di tutti $1$. Di conseguenza si vede che ogni entratadella matrice $M^2$ (prodotto righe per colonne) è $>0$. Questo vale per ogni $n$.\\
% \\
% ** Attenzione che la matrice $M$ è $n^2\times n^2$ solo nel caso "fully connected". In un caso generale è $\mathcal E \times \mathcal E$. Non posso generalizzare ponendo a zero le righe $(a,b)\notin \mathcal E$ perchè se creo righe di zeri per forza non è irriducibile. \\
% \\
% Questo metodo del bound con la monotonia al primo step e lo spectral radius può essere esteso ad altri modelli o per ottenere risultati su Belief Propagation (ad esempio lo posso usare in un modello ferromagnetico senza campi ma generale ($J_{ij}$)?)\\
% \\
% Se funziona, questo metodo può essere utile per rispondere alla domanda: la temperatura critica di un k-regolare è minore/maggiore ad esempio di un bipartito con lo stesso numero di edge? E considerare anche strutture più complesse, ad esempio due comunità fortemente connesse e poco interconnesse. A livello sociologico sarebbe interessante (chiaramente ancora no tradic closure, ma potrebbe essere studiata).
% \\
% DOBBIAMO RIvEDERE OLTRE A PHASE TRANSITION IL LEMMA CAMPI NULLI TRANNE UNO.\\
% Possiamo richiedere che M sia irriducibile e poi successivamente, in un remark, definire delle condizioni per cui sia irriducibile.\\
% 12.01 : vedere se escludere soltanto i grafi particolari è sufficiente per l'irrudicibilità.\\
% Possiamo dare il risultato della trasizione S (la 13) per M con dentro beta (e beta generico che varia da classe a classe beta ac) (raggio spettrle M maggiore e minore di 1) e poi trattare il caso di beta omogeneo dove possiamo derivare i due bound per beta critico. Definire M prima (vedere anche definizione diego stackexchange).
% \\


% altrimenti per mostrare la transizione del primo ordine (derivta prima free energy, ovvero parametro d ordine (magnetiz) discontinuo) si dovrebbe prendere S da sinistra (h-), che si può calcolare anche per simmetriasu all spins and fields flip, e far vedere che limite destro e sinistro non coincidono.

% The Curie–Weiss model exhibits two types of phase transitions:
%• When β > βc = 1/2d, the magnetization, as a function of h, is discontinuous at h = 0: there is a first-order phase transition.
%• When h = 0, the magnetization, as a function of β is continuous, but not analytic at βc: there is a continuous phase transition.
% from (https://www.unige.ch/math/folks/velenik/smbook/Curie-Weiss_Model.pdf)


% nota che sennò mi scordo: riguardo all'articolo di Collet, gli stati "discordi" m_1 m_2 <0 non sono mai globalmente stabili perchè l'energia di uno stato con m1,m2 uguali in modulo ma concordi è minori e l'entropia è la stessa. 








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% VECCHIA PROVA TEO PHASE TRANSITION
{\color{orange}
% la prova andrà dopo la prova della pressione
\begin{proof}[Old version of Proof of Theorem \ref{main: phase transition}]
    % The proof is divided in two sections. The first one focuses on the solutions of the recursion for $h=0$, identifying a value of $\beta$ below which the recursion has one unique solution at zero for any initialization and another value of $\beta$ over which a small positive initialization leads to a fixed point with all positive entries. The second section uses the results from the recursion to analyze the spontaneous magnetization of a spin on a $\mathbf{k}$-regular graph and prove its non-analyticity.\\
    \\
    % \textit{Section 1: } We consider the recursion \eqref{recursion_regular_trees} with $h=0$ for all the classes, homogeneous $\beta$ and homogeneous extra boundary field $h_*$ 
    % \begin{equation} \left\{
    % \begin{split}
    %     &\,z_a^{(b)} (s,h_*) \,= \, \sum_{c\in\mathcal E_a}\, (k_{ac}-\delta_{bc})\,F_{\beta}\big(z_c^{(a)} (s-1,h_*) \big) \,,\quad s\geq1 \\
    %     &\,z_a^{(b)} (0,h_*) \,=\, h_* \,,\quad s=0 
    % \end{split} \right.
    % \label{recursion h=0}
    % \end{equation} 
    % $\forall(a,b)\in \mathcal E$, and its fixed point $\boldsymbol{\bar z}(h_*)$.\\
    % Defining $e_a^{(b)}(s) := z_a^{(b)}(s,+\infty) - z_a^{(b)}(s,-\infty)$, we obtain
    % \begin{equation} \left\{
    % \begin{split}
    %     &\,e_a^{(b)}(s) \leq \tanh(\beta) \bigg[ \sum_{c\in\mathcal E_a} (k_{ac}-\delta_{bc}) e_c^{(a)}(s-1)\bigg] \,,\quad s\geq2 \\
    %     &\,e_a^{(b)}(1) =  \sum_{c\in\mathcal E_a} (k_{ac}-\delta_{bc}) [F_\beta(+\infty)- F_\beta(-\infty)] = 2\beta \sum_{c\in\mathcal E_a} (k_{ac}-\delta_{bc}) \,,\quad s=1
    % \end{split} \right.
    % \label{recursion e(s)}
    % \end{equation} 
    % $\forall(a,b)\in \mathcal E$, where for the bound in the first equation we have used \eqref{recursion h=0} and linearized $F_{\beta}(x_1)-F_{\beta}(x_2) \leq \max_{x\in [x_1,x_2]}F'_{\beta}(x) (x_1-x_2)$. We then rewrite \eqref{recursion e(s)} as
    % \begin{equation}
    %     \boldsymbol{e}(s) \leq \tanh(\beta) \boldsymbol{M} \boldsymbol{e}(s-1)
    % \end{equation}
    % with a suitable matrix $\boldsymbol{M}$ and vector $\boldsymbol{e}(s) = (e_a^{(b)}(s) )_{(a,b)\in \mathcal E}$. Being 
    % \begin{equation}
    %      \lVert \boldsymbol{e}(s) \rVert \leq (\tanh(\beta) \lVert \boldsymbol{M} \rVert )^{s-1} \lVert \boldsymbol{e}(1) \rVert,
    % \end{equation}
    % and $\lVert \boldsymbol{e}(1) \rVert$ finite, then 
    % \begin{equation}
    %      \tanh(\beta) \lVert \boldsymbol{M} \rVert <1
    % \label{condition norm}
    % \end{equation}
    % implies $\lim_{s\rightarrow \infty}\boldsymbol \lVert {e}(s)\rVert=\mathbf{0}$. Choosing the $\lVert \cdot \rVert_\infty$-norm, i.e. the maximum of the sums of the absolute value of the elements of the raws, we obtain that the condition \eqref{condition norm} corresponds to 
    % \begin{equation}
    %      \beta < \tanh^{-1}\bigg(   \frac{1}{\max_a k_a-1}   \bigg).
    % \label{phase transition beta critical small}
    % \end{equation}
    % Since $\lim_{s\rightarrow \infty}\lVert \boldsymbol{e}(s)\rVert_\infty =\mathbf{0}$ implies $\lim_{s\rightarrow \infty} e_a^{(b)}(s)=0 $, and applying Lemma \ref{corollary_boounds_and_monotony_H}, we obtain that the fixed point of \eqref{recursion h=0}, if existent, is unique for any initialization $h_*$. As $\boldsymbol{0}$ is always a solution of \eqref{recursion h=0}, we can conclude that for $\beta$ satisfying \eqref{phase transition beta critical small}, $\boldsymbol{\bar z}(h_*)= \boldsymbol{0}$ is the only solution of \eqref{recursion h=0} for any initialization.\\
    \\
    On the other hand, our aim is to provide a threshold of $\beta$ over which the fixed point of \eqref{recursion h=0} depends on the initialization. We first consider $n=1$: if it exists a small extra boundary field $\epsilon>0$ such that
    \begin{equation} \label{phase transition h small epsilon}
        (k-1) F_\beta(\epsilon) > \epsilon \\                                      
     \end{equation}
    corresponding to the condition \eqref{condition_H_small} strict, then by Proposition \ref{lemma_uniqueness} 
    \begin{equation}
        \boldsymbol{\bar z}(h_*) = \boldsymbol{\bar z^+} \quad \quad \forall\;\; h_*\geq \epsilon
    \end{equation}
    where $\boldsymbol{\bar z^+} = (z_a^{(b)+}\in[\epsilon,+\infty))_{(a,b)\in \mathcal E}$, the unique fixed point with entries $\geq \epsilon$.
    By Taylor expanding \eqref{phase transition h small epsilon}
    \begin{equation}
     \begin{split}                                     
         &(k-1) (F'_\beta(0)\epsilon +    O(\epsilon^2)) > \epsilon        \\                                   
         &\tanh(\beta) > \frac{1}{k-1} +   O(\epsilon) 
     \end{split}         
     \end{equation}
     we obtain a condition on $\beta$ over which any small $\epsilon$ satisfies \eqref{phase transition h small epsilon}, namely
     \begin{equation}\label{beta critical n=1}
         \beta>\tanh^{-1}\bigg(\frac{1}{k-1}\bigg)
     \end{equation}
     Extending to $n>1$, \eqref{phase transition h small epsilon} becomes 
     \begin{equation} 
        (\min_{a=\{1,\ldots,n\}}k_a-1) F_\beta(\epsilon) > \epsilon \\                                      
     \end{equation}
     and thus we get
     \begin{equation}\label{beta critical n>1 above which ferro solution}
         \beta>\tanh^{-1}\bigg(\frac{1}{\min_{a}k_a-1}\bigg)
     \end{equation}  
     as a threshold of $\beta$ over which the recursion \eqref{recursion h=0} has a fixed point with all positive entries, reached by any strictly positive initialization.\\
     \\
     \\
     \\
    %  \textit{Section 2:} Now we consider the Ising model on a $\mathbf k$-regular graph and specifically \eqref{S zero fields function}, where the limit with respect to $N$ in $L^r-$norm is given by the expression \eqref{eq: main magnetization} (Theorem \ref{main:magnetization}).\\
    %  At $h>0$, $\boldsymbol{\bar z}=\boldsymbol{\bar z}(\beta,h)$ is the only solution with all positive entries of the fixed point equation
    %  \begin{equation}
    %          \bar z_a^{(b)} \,=\, h + \sum_{c\in \mathcal E_a} (k_{ac}-\delta_{bc})\, F_{\beta}\big(\bar z_c^{(a)}\big)\,, \quad (a,b)\in\mathcal E \,.
    % \label{fixed point eq with field}
    %  \end{equation}
    % We consider the limit $\lim_{h\to 0^+}\boldsymbol{\bar z}(\beta,h)\,$, reached with decreasing monotonicity by Lemma \ref{corollary_boounds_and_monotony_H}. From \eqref{fixed point eq with field}, for the continuity of the function $F$, $\lim_{h\to 0+}\boldsymbol{\bar z}(\beta,h)\,$ is a solution of 
    %  \begin{equation}
    %          \tilde z_a^{(b)} \,=\, \sum_{c\in \mathcal E_a} (k_{ac}-\delta_{bc})\, F_{\beta}\big( \tilde z_c^{(a)}\big)\,, \quad (a,b)\in\mathcal E\,.
    % \label{fixed point eq no field}
    %  \end{equation}    
    % i.e. of \eqref{recursion h=0}. From the results above, for $\beta < \tanh^{-1}(\frac{1}{\max_{a}k_a-1})$ \eqref{recursion h=0} has a unique and null solution, thus $\lim_{h\to 0+}\boldsymbol{\bar z}(\beta,h)=\boldsymbol{0}$. If instead  $\beta > \tanh^{-1}(\frac{1}{\min_{a}k_a-1})$, the recursion \eqref{recursion h=0} has also one strictly positive solution $\boldsymbol{\bar z^+}(\beta)$. \\
    % At $h>0$, by Theorem \ref{main:magnetization} $\boldsymbol{\bar z}(\beta,h)= \lim_{s\rightarrow\infty}\bar z(s)$, where in particular we can fix the initialization of the recursion as
    %  \begin{equation} \left\{
    %  \begin{split}
    %     &\,z_a^{(b)} (s,h_*) \,= \,h\;+\; \sum_{c\in\mathcal E_a}\, (k_{ac}-\delta_{bc})\,F_{\beta}\big(z_c^{(a)} (s-1,h_*) \big) \,,\quad s\geq1 \\
    %     &\,z_a^{(b)} (0,h_*) \,=\, \bar z_a^{(b)+}(\beta) \,,\quad s=0 
    % \end{split} \right.
    % \label{recursion h>0}
    % \end{equation}
    % $\forall(a,b)\in \mathcal E$.\\    
    % By the monotonicity of $F$, the positivity of $h$ and the fact $z_a^{(b)+}(\beta)>0$, it is easy to verify by induction that
    % \begin{equation}
    %     \bar z_a^{(b)}(\beta,h) \,\geq\, \bar z_a^{(b)+}(\beta)\,, \quad (a,b)\in\mathcal E \;.
    % \end{equation} 
    % Taking $h\to0^+$
    % \begin{equation}
    % \lim_{h\to0^+}\bar z_a^{(b)}(\beta,h) \,\geq\, \bar z_a^{(b)+}(\beta)\,, \quad (a,b)\in\mathcal E 
    % \end{equation}
    % and eventually considering that \eqref{fixed point eq no field} has no other solutions with entries greater than $\bar z_a^{(b)+}(\beta)$, than it must be
    % \begin{equation}
    %     \lim_{h\to0^+}\bar z_a^{(b)}(\beta,h) \,=\, \bar z_a^{(b)+}(\beta)\,, \quad (a,b)\in\mathcal E ,
    % \end{equation}
    % completing the proof.
    
% in teoria sarebbe z(beta, h, h_*), dove h_* sono le condizioni al bordo
% sto prendendo z(beta, h=0, h_*>0) come condizioni iniziali della ricorsione h>0
% puoi prendere tranquillamente il limite del punto fisso? Cioè dire che se la disuguaglianza vale per h>0 alloravale anche al limite 
\end{proof}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% vecchie considerazioni remark e prove phase transition, anche prova di diego
{\color{blue}Se funziona tutto, direi di far diventare la remark seguente un teorema nella sezione main.}
\begin{remark}
     In the homogeneous case of only one class ($n=1$, $\beta_{11}=\beta$, $k_{11}=k$) and zero external field, Proposition \ref{lemma existence fixed point H_small H_big} provides a sufficient condition on $\beta$ for the existence of at least one strictly positive fixed point of the recursion \eqref{recursion_regular_trees}. Taking $h_*^{small}=\epsilon>0$, the condition (\ref{condition_H_small}) reads
     \begin{equation}
     \begin{split}
         &(k-1) F_\beta(\epsilon) \geq \epsilon \\                                      
         &(k-1) (F'_\beta(0)\epsilon +    O(\epsilon^2)) \geq \epsilon        \\                                   
         &\tanh(\beta) \geq \frac{1}{k-1} +   O(\epsilon) 
     \end{split}         
     \end{equation}
     If $\beta>\tanh^{-1}(\frac{1}{k-1})=: \beta_+$, then every $\epsilon$ sufficietly small verifies the previous condition. {\color{blue}Quindi per la Proposizione \ref{lemma existence fixed point H_small H_big}, la ricorsione \eqref{recursion_regular_trees} ha un punto fisso con componenti strettamente positive $\bar z_a^{(b)}(\epsilon)\geq\epsilon$.}  
     
     % Thus, we derived an upper bound $\beta^+_c$ for the critical inverse temperature (a value of the inverse temperature after which the couple of ferromagnetic solutions is surely present). The upper bound coincides, in this case, with the critical value found by statistical physics calculations for a homogeneous Ising model in random $k$-regular graphs \cite{leone2002ferromagnetic} {\color{blue} citare anche Dembo-Montari}
\end{remark}
{\color{red}Estendere il punto precedente ad un albero $\mathbf{k}$-regolare con più classi e $\beta$ omogeneo.}\\

{\color{purple} 
Applicando le stesse considerazioni sopra, la condizione di monotonia deve essere verificta per ogni equazione del sistema () e quindi è sufficiente che sia verificata per quella con $k$ minore. Si trova quindi
$$\tanh(\beta) \geq \frac{1}{\min_a \sum_{c\in \mathcal E_a} (k_{ac}-\delta_{bc})} +   O(\epsilon) = \frac{1}{\min_a k_a-1} +   O(\epsilon) $$
Ovvero 
$$\beta_+ =  \tanh^{-1}\bigg(\frac{1}{\min_a k_a-1} \bigg) $$
valore di $\beta$ oltre il quale esiste sicuramente almeno una soluzione strettamente positiva della ricorsione.}\\

{\color{red} Dall'altra parte cerchiamo un valore di $\beta$ sotto il quale il punto fisso non dipende dall'inizializzazione della ricorsione, e quindi è unico e zero (poichè è sempre punto fisso).}\\

{\color{purple} Estendendo il Lemma di Dembo per il multi-regular, definendo $e_a^{(b)}(s) := z_a^{(b)}(s,+\infty) - z_a^{(b)}(s,-\infty)$ ho che 
$$e_a^{(b)}(s) \leq \tanh(\beta) \bigg[ \sum_{c\in\mathcal E_a} (k_{ac}-\delta_{bc}) e_c^{(a)}(s-1)\bigg]   \quad \quad \forall (a,b) \in \mathcal E$$
inizializzata da
$$e_a^{(b)}(1) =  \sum_{c\in\mathcal E_a} (k_{ac}-\delta_{bc}) [F_\beta(+\infty)- F_\beta(-\infty)] = 2\beta \sum_{c\in\mathcal E_a} (k_{ac}-\delta_{bc}) \quad \quad \forall (a,b) \in \mathcal E$$
Scrivo la ricorsione in forma matriciale: per scriverla in forma compatta, assumo che $e_a^{(b)}(s)=0$ per ogni $(a,b)\notin \mathcal E$
$$\boldsymbol{e}(s) \leq \tanh(\beta) \boldsymbol{M} \boldsymbol{e}(s-1)$$
dove $\boldsymbol{e}(s) := ( e_1^{(1)}(s), e_1^{(2)}(s),...,e_1^{(n)}(s),e_2^{(1)}(s),\ldots,\ldots,e_n^{(n)}(s)) $ and $M_{ab}=  $ (si può scrivere). Ho che
$$ \lVert \boldsymbol{e}(s) \rVert \leq (\tanh(\beta) \lVert \boldsymbol{M} \rVert )^t \lVert \boldsymbol{e}(0) \rVert$$
quindi se $\tanh(\beta) \lVert \boldsymbol{M} \rVert <1$, $\lim_{s\rightarrow \infty}\boldsymbol \lVert {e}(s)\rVert=\mathbf{0} $ e il punto fisso è unico. Scelgo $\lVert \boldsymbol{M} \rVert = \max_{i}\sum_{j=1}^{n^2}|m_{ij}|$ (norma massimo della somma delle righe) e vedo che la condizione sopra è verificata per $\beta<\beta_0$ dove
$$\beta_0 := \tanh^{-1}\bigg(   \frac{1}{\max_a k_a-1}   \bigg)$$
}

{\color{red}Ora cerchiamo di applicare i risultati al grafo, servendoci dei risultati con campi positivi.}\\
{\color{red}Q: Possiamo prendere anche l'unicità della soluzione strettamente positiva dalla Proposizione \ref{lemma_uniqueness} ? Possiamo dire che è raggiunta da qualsiasi inizializzazione positiva della ricorsione? }\\
{\color{purple} Penso di sì, anche se a questo punto del testo non abbiamo ancora i risultati per l'unicità.}\\

{\color{red} C'è una transizione di fase (punto di non analiticità) sul grafo? Sì.} {\color{purple}Ora cerchiamo di sfruttare i risultati sopra per l'estensione al grafo.*}

{\color{blue} Consideriamo il modello di Ising \eqref{...} sul grafo random $\mathbf k$-regolare $G_N$ con campo esterno $h$ e temperatura inversa $\beta$ omogenei. La \textit{magnetizzazione spontanea} di uno spin $\sigma_i$, $i\in C_a$ è:
\begin{equation} \label{eq: spontaneous}
    S_a(\beta) :=\, \lim_{h\to 0+}\lim_{N\to\infty}\langle \sigma_i\rangle_{G_N,\beta,h} \,=\, \lim_{h\to 0+} \tanh\Big( h_a + \sum_{b\in\mathcal E_a} k_{ac}\, F_{\beta_{ac}}\big(\bar{z}_c^{(a)}\big) \Big)
\end{equation}
dove il limite rispetto ad $N$ è in norma $L^r(\mathbb P)$ ed è dato dall'espressione \eqref{eq: main magnetization} (teorema \ref{...}). Ad $h>0$, $\boldsymbol{\bar z}=\boldsymbol{\bar z}(\beta,h)$ è l'unica soluzione con componenti positive ($\geq h$) dell'equazione di punto fisso
\begin{equation} \label{eq:fix point h}
    \bar z_a^{(b)} \,=\, h_a + \sum_{c\in \mathcal E_a} (k_{ac}-\delta_{bc})\, F_{\beta_{ac}}\big(\bar z_c^{(a)}\big)\,, \quad (a,b)\in\mathcal E \,.
\end{equation}
Consideriamo il limite $\lim_{h\to 0+}\boldsymbol{\bar z}(\beta,h)\,$, raggiunto con monotonia decrescente (proposition \ref{...}). Dalla \eqref{eq:fix point h}, per continuità di $F$, esso è una soluzione di 
\begin{equation} \label{eq:fix point h=0}
    \tilde z_a^{(b)} \,=\, \sum_{c\in \mathcal E_a} (k_{ac}-\delta_{bc})\, F_{\beta_{ac}}\big( \tilde z_c^{(a)}\big)\,, \quad (a,b)\in\mathcal E\,.
\end{equation}
Se $0<\beta\leq\beta_c$, l'equazione \eqref{eq:fix point h=0} ha una sola soluzione (remark \ref{...}), che è quella nulla. Perciò $\lim_{h\to 0+}\boldsymbol{\bar z}(\beta,h)=\boldsymbol{0}$.\\
Se invece $\beta>\beta_c$, l'equazione \eqref{eq:fix point h=0}, oltre alla soluzione nulla, ha una (unica?) soluzione con componenti strettamente positive (remark \ref{...}) che indichiamo con $\boldsymbol{\bar z}^+(\beta)$. 
{\color{purple}* in generale (vedi su) troviamo $\beta_{pos}=\tanh^{-1}(\frac{1}{\min_a k_a -1}$ e $\beta_{0}=\tanh^{-1}(\frac{1}{\max_a k_a -1}$, quindi $\beta_{pos}\geq \beta_0$. $\beta_{pos} = \beta_0 := \beta_c$ solo nel caso di una sola classe (il caso a più classi $k_a=k_b=...$ è equivalente a quello a una classe. Quindi credo che si debba modificare la frase sopra.}\\
Ora, quando $h>0$ per il teorema \ref{...} $\boldsymbol{\bar z}(\beta,h) = \lim_{s\to\infty}\boldsymbol{ z}(s)$, dove in particolare possiamo scegliere
\begin{equation} \label{eq:recursion z} \begin{cases}
    z_a^{(b)}(s) \,=\, h_a + \sum_{c\in \mathcal E_a} (k_{ac}-\delta_{bc})\, F_{\beta_{ac}}\big( z_c^{(a)}(s-1)\big)\,,\quad s\geq1 \\
    z_a^{(b)}(0) \,=\, \bar z_a^{(b)+}(\beta)
\end{cases} \,, \ (a,b)\in\mathcal E\,.
\end{equation}
%E inoltre $\boldsymbol{\bar z}^+ = \lim_{s\to\infty}\boldsymbol{ z}^+(s)$ dove
%\begin{equation} \label{eq:recursion z+} \begin{cases}
%    z_a^{(b)+}(s) \,=\, \sum_{c\in \mathcal E_a} (k_{ac}-\delta_{bc})\, F_{\beta_{ac}}\big( z_c^{(a)+}(s-1)\big)\,,\quad s\geq1 \\
%    z_a^{(b)+}(0) \,=\, \epsilon >0
%\end{cases} \,, \ (a,b)\in\mathcal E\,.
%\end{equation}
%Inizializzando entrambe le ricorsioni \eqref{eq:recursion z}, \eqref{eq:recursion z+} allo stesso $\epsilon>0$,
Usando la monotonia di $F$, la positività di $h$ ed il fatto che $\boldsymbol{\bar z}^+(\beta)$ è soluzione di \eqref{eq:fix point h=0}, è facile verificare per induzione su $s$ che
\begin{equation}
\bar z_a^{(b)}(\beta,h) \,\geq\, \bar z_a^{(b)+}(\beta)\,, \quad (a,b)\in\mathcal E \;.
\end{equation} 
Mandando $h\to0+$
\begin{equation}
\lim_{h\to0+}\bar z_a^{(b)}(\beta,h) \,\geq\, \bar z_a^{(b)+}(\beta)\,, \quad (a,b)\in\mathcal E \,.
\end{equation}
Non essendoci altre soluzioni di \eqref{eq:fix point h=0} con componenti maggiori di $\bar z_a^{(b)+}(\beta)$, deve valere $\lim_{h\to0+}\boldsymbol{\bar z}(\beta,h) \,=\, \boldsymbol{\bar z}^{+}(\beta)\,$.\\
In conclusione, sostituendo in \eqref{eq: spontaneous} i limiti ottenuti, troviamo
\begin{equation}
    S_a(\beta) \,=\, \begin{cases}
        \,0 &\textrm{,\,if }0<\beta\leq\beta_c \\
        \,\tanh\Big( \sum_{b\in\mathcal E_a} k_{ac}\, F_{\beta_{ac}}\big(\bar{z}_c^{(a)+}\big) \Big)>0 &\textrm{,\,if }\beta>\beta_c 
    \end{cases}
\end{equation}
perciò $S_a$ non è una funzione analitica di $\beta$.
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% vecchie versioni remark campi nulli tranne uno
    %
    %As $\mathbf{k}$ is irreducible, and the doubled nodes are connected in the same way of the original ones, the newtork is connected, meaning that for any couple of nodes there exists a (non-backtracking) path connecting them. If we indicate with $P_{a}(s')$ the set of paths starting from $a$ of lengths up to $s'$, we know that there exists a finite length for which these paths touch every class, i.e. $N(P_{a}(s'^*))=\{1,\ldots,n\}$.\\
    %
    %%Now, we claim that for every $s\geq s_0$ there exists $s'\geq s$ such that
    %%\begin{equation}
    %%     \mathcal C\big(P_{a}^{(b)}(s')\big) \,\supseteq\, \mathcal C\big(P_a(s)\big) \,.
    %%\label{eq all classes}
    %%\end{equation}
    %%It will follow $\mathcal C\big(T_a^{(b)}(s')\big) = \mathcal C\big(P_{a}^{(b)}(s')\big) = \{1,\dots,n\}$, completing the proof of the present lemma.
    %%In order to prove claim \eqref{eq all classes} we consider three cases:
    %%\begin{itemize}
    %%    \item[i)] if $k_{ab}\geq2$, then trivially $P_a^{(b)}(s)=P_a(s)$;
        %\item[ii)] if $k_{ab}=1$, $k_{aa}\geq1$, then a walk starting by $aab\dots$ is allowed in $P_a^{(b)}$, hence $P_a^{(b)}(s+1)\supseteq\{a\}\times P_a(s)$ and \eqref{eq all classes} follows;
    %%    \item[iii)] if $k_{ab}=1$, $k_{aa}=0$, and $ab$ is not a cut-edge in the direct graph $\mathcal G$ (i.e., $\mathcal G$ remains strongly connected by removing $ab$), then ...
    %%    \item[iv)] if $ab$ is a cut-edge of $\mathcal G$, $k_{ab}=1$, $k_{aa}=0$, since by hypothesis $k_a\geq2$ there exists $c\neq b$ such that $k_{ac}\geq1$, hence a walk starting by $ac\dots$ is allowed in $P_a^{(b)}$. Since $ab$ is a cut-edge, there is a walk of $P_a$ that goes back to $a$ without touching $b$ %Therefore $P_a^{(b)}(s')\supseteq\{a\}\times P_c^{(a)}(s'-1)$.
    %%\end{itemize}
    
    %For $P^*_{a(b)}$ this may in principle not be true, due to the restriction on the first step, but we show that $\exists s^*,s'^*$ finite such that 
    %\begin{equation}
    %     N(P^*_{a(b)}(s^*)) = N(P_a(s'^*)) = \{1,\ldots,n\}
    %\label{eq all classes}
    %\end{equation}
    %by exploring all the possible cases:
    %\begin{itemize}
        %\item \textbf{$ab$ is not red:}  then $N(P^*_{a(b)}(s)) = N(P_a(s))$ and \eqref{eq all classes} follows trivially.
        %\item \textbf{$ab$ is red but $aa$ exists:}  then $aab$ is allowed to reach $b$ and \eqref{eq all classes} follows.
        %\item \textbf{$ab$ is red, $aa$ does not exist but $ab$ is not a bridge} (an edge whose deletion disconnects the graph): as $ab$ is not a bridge, there exists a set of non-backtracking (always allowed) paths that touch all the classes without using the edge $ab$, proving $N(P^*_{a(b)}(s^*)) = \{1,\ldots,n\}$, thus \eqref{eq all classes}.   
        %\item \textbf{$ab$ is red, $aa$ does not exist and $ab$ is a bridge: } as $k_a\geq 2$, it must exist $c\in E_a, c\neq b$. We claim that there exists at least a path that starts with $ac$ and goes back to $a$ through $c'a$, $c'\neq b$, so whose next step can be $ab$ thus proving \eqref{eq all classes}. The existence of such path is proved noticing that or $ac...c'a$ includes a loop (it would never backtrack so it is always allowed), else it reaches a leaf $f$, where it it easy to see that it can always backtrack ($k_f=k_{ff}+k_{fg}\geq 2$), thus such path would be $ac...gfg...ca$.
    %\end{itemize}
%
% {\color{brown} 
%     We build the network of classes with nodes $\{1,\ldots,n\}$ and $a\neq b$ connected if $k_{ab}\geq 1$ (and thus $k_{ba}\geq 1$). As $\mathbf{k}$ is irreducible, the graph is connected. Indicating with $\partial a$ the neighbours of $a$ ($\partial a \equiv \mathcal E_a$), we define
%     \begin{itemize}
%         \item $P^{NB}_{a}$ the collection of non-backtracking finite paths starting from $a$
%         \item $P^{NB}_{a(b)}$, $b\in \partial a$, the collection of non-backtracking finite paths starting from $a$ with any first step but the edge $ab$
%         \item $P^{NB}_{ab}$ the collection of non-backtracking finite paths starting from $a$ with first step the edge $ab$
%     \end{itemize}
%     Denote with $N(P^{NB}_{a})$,$N(P^{NB}_{a(b)})$ and $N(P^{NB}_{ab})$ the sets of nodes (classes) touched by the corresponding collection of paths. Being $P^{NB}_{a(b)} \cup P^{NB}_{ab} = P^{NB}_{a}$, also $N(P^{NB}_{a(b)}) \cup N(P^{NB}_{ab}) = N(P^{NB}_{a})$. As the graph is connected, $ N(P^{NB}_{a}) = \{1,\ldots,n\}$.\\
%     \\
%     Consider the same graph, but with directed edges (and no self-edges) and coloring in red the edges $cd$ with $k_{cd}=1$ and $k_{cc}=0$. Consider the collections of all possible paths of lengths up to $s$, $P^{*}_{a(b)}(s)$, $b\in \partial a$, that start from $a$ with any first step but the edge $ab$ if it is red and can be also backtracking, with the exception that they cannot walk $dcd$ if $cd$ is red. Note that 
%     \begin{equation}
%         N(T_a^{(b)}(s)) = N(P^{*}_{a(b)}(s))
%     \end{equation}
%     where $N(T_a^{(b)}(s))$ is the set of classes in $T_a^{(b)}(s)$. Our aim is to prove that $\exists s,s' >0$ finite such that
%     \begin{equation}
%         N( P^{*}_{a(b)}(s'+s)) \supseteq  N(P^{NB}_{a(b)}(s)) \cup N(P^{NB}_{ab}(s)) = N(P^{NB}_{a}(s)) = \{1,\ldots,n\}
%     \label{set equivalence_tobe proved}
%     \end{equation}
%     For proving \eqref{set equivalence_tobe proved}, we consider three cases:
%     \begin{itemize}
%         \item If $ab$ is not red, $   P^{NB}_{a(b)}(s) \cup P^{NB}_{ab}(s) = P^{NB}_{a}(s)  \subseteq P^{*}_{a(b)}(s'+s))  $ and \eqref{set equivalence_tobe proved} is proved.\\
%         \\
%         If $ab$ is red, then there exists $c\in \partial a, c\neq b,a$, as $k_a\geq 2$ and $k_{aa}=0$. We have the following sub-cases:
%         \item If there is a loop $acde...ba$, the cancellation of the edge $ab$ ($ba$) does not preclude the connectivity of the graph, so $\exists s,s'$ such that 
%         $$  N(P^{NB}_{a}(s)) = N( P^{*}_{a(b)}(s'+s)) = \{1,\ldots,n\}  $$
%         \item We consider the case in which from $ac$ there is no loop ending in $ba$. We notice that, as since $k_f\geq2$ $\forall f$ there is no leaf $f$ connected through a red edge $fg$, the path can always backtrack in any leaf. The path $acdef...$ is either a loop going back to $a$ through $c'a$ ($c\neq c,b$) or it backtracks at a leaf coming back to $a$ through $ca$. Indicating with $s'$ the length of the shortest of the paths returning to $a$ through any $ca$, $c\neq b$, we have that 
%         $$ P^{NB}_{ab}(s)  \subseteq   P^{*}_{a(b)}(s'+s)  $$
%         Finally, noticing that $ P^{NB}_{a(b)}(s) \subseteq P^{*}_{a(b)}(s'+s)$, 
%         $$  P^{NB}_{a(b)}(s) \cup P^{NB}_{ab}(s) \subseteq P^{*}_{a(b)}(s'+s)   $$
%         and so \eqref{set equivalence_tobe proved} is proved.
%     \end{itemize}   

==> trees/existence.tex <==
\begin{corollary}
    For any $i,j$ and $t$, for $z_i^{(j)}(d,T_v(t),H)$, $d=1,...,t-1$ we have that
    \begin{equation}
        h_i-\sum_k (k_{ik}-\delta_{jk}) \beta_{ik} \leq z_i^{(j)}(d,T_v(t),H)  \leq  h_i + \sum_k (k_{ik}-\delta_{jk}) \beta_{ik}
    \label{bounds}    
    \end{equation}
    Moreover, $H \longmapsto z_i^{(j)}(d,T_v(t),H)$ for any $d=1,...,t-1$ is monotonic non-decreasing.
\label{corollary_boounds_and_monotony_H}
\end{corollary}

\begin{proof}
    The proof of the first statement comes directly from the application of the recursion (\ref{recursion_regular_trees}), noting that $z^{(j)}_w(d,T_v(t),H)$ is monotonic with respect to all $z^{(w)}_{w'}(d+1,T_v(t),H)$, $w'=1,...,n$. Indeed
    \begin{equation}
        \frac{\partial z^{(j)}_w(d,T_v(t),H)}{\partial z^{(w)}_{w'}(d+1,T_v(t),H)} = C_{jww'} \frac{\partial F_{\beta_{ww'}}( z^{(w)}_{w'}(d+1,T_v(t),H))}{\partial  z^{(w)}_{w'}(d+1,T_v(t),H)} 
    \label{derivatives_recursion}
    \end{equation}
    with a coefficient $C_{jww'}\geq0$, and the monotonicity follows from 
    \begin{equation}
         \frac{\partial F_\beta(x)}{\partial x} = \frac{\tanh(\beta)}{1+(1-\tanh^2(\beta))\sinh^2(x)} \geq 0 \;\;\;\;\;\; \forall \; x\in \Real
    \label{F_beta_first_derivative}
    \end{equation}
   Thus, for the lower and upper bounds we take the lowest and largest possible values of each $z^{(w)}_{w'}(d+1,T_v(t),H)$ for $w'=1,...,n$ ( respectively $z^{(w)}_{w'}(d+1,T_v(t),H)\rightarrow -\infty$ and $z^{(w)}_{w'}(d+1,T_v(t),H)\rightarrow +\infty$; notice that these extremes can be reached only at the boundary, i.e., for $d+1=t$), ending up with (\ref{bounds}).\\
   \\
   The second statement, i.e., the monotonic behaviour with respect to the boundary fields, is a direct consequence of the FKG inequalities: considering the magnetization $\Tilde{m}_i^{(j)}(d)$ under the Ising measure restricted on the subgraph $T_{i(j)}(\mathbf{k},d)$, we recall that $z_i^{(j)}(d,T_v(t),H) \equiv \tanh^{-1}\bigg( \Tilde{m}_i^{(j)}(d) \bigg)$, so taking the variation with respect to the homogeneous field $H$ applied at the boundary we have
   $$\frac{d z_i^{(j)}(d,T_v(t),H)}{d H} = \frac{\partial z_i^{(j)}(d,T_v(t),H)}{\partial \Tilde{m}_i^{(j)}(d)} \frac{\partial \Tilde{m}_i^{(j)}(d)}{\partial h'_g} \frac{d h'_g}{d H}$$
   for $g\in V_*$ (the boundary of $T_v(t)$), so $h'_g = h_g + H $. It is easy to see that $\frac{\partial z_i^{(j)}(d,T_v(t),H)}{\partial \Tilde{m}_i^{(j)}}> 0$, moreover $\frac{d h'_g}{d H}=1$ . By the FKG inequality, $\frac{\partial \Tilde{m}_i^{(j)}(d)}{\partial h'_g}\geq0$. Thus, $\frac{\partial z_i^{(j)}(d,T_v(t),H)}{\partial H}\geq0$, concluding the proof.
\end{proof}


% \begin{remark}
%     Being $\bar{z}_i^{(j)}(H) = \lim_{t\rightarrow\infty}z_i^{(j)}(1,T_v(t),H)$ the fixed point of the recursion, if existing, it is monotonic non-decreasing with respect to the added field at the boundary $H$.
% \end{remark}

\vskip 2 cm
The following Lemma exploits the monotonicity of $H \longmapsto z_i^{(j)}(d,T_v(t),H)$ to prove the existence of at least one fixed point for a specific interval of added fields at the boundary.
\vskip 2 cm


\begin{lemma}
    If
    \begin{equation}
         \sum_k (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(h_k+H_{small})\geq H_{small} \;\;\;\;\;\;\;\; \forall \;i,j=1,...,n
    \label{condition_H_small}
    \end{equation}
   for a $H_{small}$, then there exists a fixed point of the recursion $\boldsymbol{\bar{z}}(H_{small})$ with $\bar{z}_i^{(j)}(H_{small})\geq h_i + H_{small} $, $\forall i,j$. \\
   At the same time if for another $H_{big}>H_{small}$, not necessairly finite, such that
    \begin{equation}
        \sum_k (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(h_k+H_{big})\leq H_{big} \;\;\;\;\;\;\;\; \forall \;i,j
    \label{condition_H_big}
    \end{equation}
    then there exists a fixed point of the recursion $\boldsymbol{\bar{z}}(H_{big})$ with $\bar{z}_i^{(j)}(H_{big})\leq h_i + H_{big}$, $\forall i,j$. \\
    Moreover, for $H\in[H_{small},H_{big}]$ and large $t$, $z_i^{(j)}(d,T_v(t),H) \in [\bar{z}_i^{(j)}(H_{small}),\bar{z}_i^{(j)}(H_{big})]$,  $\forall i,j$.
\label{lemma existence fixed point H_small H_big}
\end{lemma}

\begin{proof}
    For the proof, we use the monotonic behaviour of $z_i^{(j)}(d,T_v(t),H)$ with respect to the inclusion of a new (boundary) generation, so considering a tree $T_v(t+1)$, keeping the same homogeneous added field $H$ at the boundary. \\
    From 
    $$\frac{\partial z^{(j)}_w(d,T_v(t),H)}{\partial z^{(w)}_{w'}(d+1,T_v(t),H)} \geq 0 \;\;\;\;\;\;\;\;\;\; \forall \; j,w,w',t,H \;\;\;\;\;\;\;\; \; d=1,...,t-1$$
    (see eq. (\ref{derivatives_recursion}) and (\ref{F_beta_first_derivative})), it follows that if  
    \begin{equation}
        z_i^{(j)}(d=t,T_v(t+1),H) \geq z_i^{(j)}(d=t,T_v(t),H) \;\;\;\;\;\;\;\forall \; i,j
    \label{Hsmall_inclusion_generation_inequality}
    \end{equation}
    so equivalently if
    \begin{equation}
         h_i + \sum_k (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(h_k+H) \geq h_i + H
    \label{analogous_condition_H_small}
    \end{equation}
    then 
    $$z_i^{(j)}(d,T_v(t+1),H) \geq z_i^{(j)}(d,T_v(t),H) \;\;\;\;\;\;\;\forall \; i,j$$
    for all $d$, so we say that $z_i^{(j)}(d,T_v(t),H)$ is monotonic non-decreasing with respect to the inclusion of a new generation ($t\rightarrow t+1$), so, iterating, with respect to $t$. Note that (\ref{analogous_condition_H_small}) corresponds to (\ref{condition_H_small}), to be satisfied with a choice of the added field at the boundary $H_{small}$.\\
    \\
    Reasoning in an analogous way, one finds that if the condition (\ref{condition_H_big}) is satisfied for a $H_{big}$, then 
    \begin{equation}
        z_i^{(j)}(d=t,T_v(t+1),H_{big}) \leq z_i^{(j)}(d=t,T_v(t),H_{big}) \;\;\;\;\;\;\;\forall \; i,j
    \label{Hbig_inclusion_generation_inequality}
    \end{equation}
    and so each $z_i^{(j)}(d,T_v(t),H_{big})$ is monotonic non-increasing with respect to $t$.\\
    \\
    Once found $H_{big}, H_{small}$, with $H_{small}<H_{big}$, as each $z_i^{(j)}(d,T_v(t),H)$ for $d<t$ stands within two finite bounds (Corollary \ref{corollary_boounds_and_monotony_H}), and moreover for $H_{big}, H_{small}$ is respectively non-increasing and non-decreasing with respect to $t$, then for $t\rightarrow\+\infty$ and $d$ finite, the two curves $z_i^{(j)}(d,T_v(t),H_{big})$ and $z_i^{(j)}(d,T_v(t),H_{small})$ must approach respectively from the top and from the bottom two potentially different fixed points, respectively $\bar{z}_i^{(j)}(H_{big})$ and $\bar{z}_i^{(j)}(H_{small})$. The latter fixed points are independent of $d$, as $z_i^{(j)}(d,T_v(t),H) = z_i^{(j)}(d+\gamma,T_v(t+\gamma),H)$. Moreover, as $z_i^{(j)}(d,T_v(t),H)$ is monotonic non-decreasing with respect to $H$ (Corollary \ref{corollary_boounds_and_monotony_H}), then $\bar{z}_i^{(j)}(H_{big})\geq\bar{z}_i^{(j)}(H_{small})$. For the same reason, at large $t$ $z_i^{(j)}(d,T_v(t),H)$ for $H\in[H_{small},H_{big}]$ must stay within the bounds $[\bar{z}_i^{(j)}(H_{small}),\bar{z}_i^{(j)}(H_{big})]$.
    %monotonia rispetto a inclusione di nuova generazione + bounds del punto fisso + mootonia rispetto  H (per vedere che sta nel bound)
\end{proof}

\begin{corollary}
    If all the external fields of the classes are non-negative, there exists at least one fixed point of the recursion with all non-negative entries. 
\end{corollary}

\begin{proof}
    If all the external fields of the classes are non-negative, the condition (\ref{condition_H_small}) is satisfied by $H_{small}=0$. This means that, according to the Lemma, there exists at least one fixed point of the recursion with $\bar{z}_i^{(j)}(H_{small})\geq h_i$, so all non-negative entries. 
\end{proof}

\begin{remark}
    In the case of all non-negative fields, the proof of Lemma \ref{lemma existence fixed point H_small H_big}, specifically the conditions for the monotonic behaviours of the magnetizations with repect to the inclusion of a new generation, can be performed in an alternative way, setting $H_{small}=0$ (free boundary conditions) and $H_{big}=+\infty$ (positive boundary conditions), by using the GKS inequalities:
\label{remark_proof_GKS}
\end{remark}
\begin{proof}
    Consider a $\mathbf{k}$-regular tree of depth $t$ and root $v$, $T_v(t)$, with all positive boundary conditions obtained (equivalently) by fixing the fields of the spins at the boundary to $+\infty$. Consider also a subtree with the same root with a further generation $T'_v(t+1)$ with positive infinite fields not only at the last generation, but also at the generation $t$. Intuitively, the magnetizations at the root are equivalent for $T_v(t)$ and $T'_v(t+1)$. Now, we remove from $T'_v(t+1)$ the fields of the generation $t$, leaving only those in $t+1$. Doing so, we obtained exactly what we considered as $T_v(t+1)$ with all positive boundary conditions (infinite fields). As we only removed fields, the GKS theorem holds and for any magnetization in the subree (any $d$)
    $$z_i^{(j)}(d,T_v(t+1),\infty) \leq z_i^{(j)}(d,T'_v(t+1),\infty) \;\;\;\;\;\;\;\forall \; i,j$$
    Considering that $z_i^{(j)}(d,T'_v(t+1),\infty) = z_i^{(j)}(d,T_v(t),\infty)$, we have found (\ref{Hbig_inclusion_generation_inequality}) for $H_{big}=\infty$.\\
    \\
    For the free boundary conditions, consider a subtree with the same root as before $T_v(t)$ with all free boundary conditions (in the sense that there is no added field, $H=0$). Consider also a tree $T'_v(t+1)$ with no added field at the last two generations and no edges among the spins of the last two generations. Intuitively, the magnetizations at all subtrees are equivalent for $T_v(t)$ and $T'_v(t+1)$ (the nodes in the generation $t+1$ are isolated). Now, we add to $T'_v(t+1)$ the missing edges among the last two generation. Doing so, we obtained exactly what we considered as $T_{t+1}$ with all free ($H=0$) boundary conditions. As we only added edges, the GKS theorem holds and 
    $$z_i^{(j)}(d,T_v(t+1),0) \geq z_i^{(j)}(d,T'_v(t+1),0) \;\;\;\;\;\;\;\forall \; i,j$$
    Considering that $z_i^{(j)}(d,T'_v(t+1),0) = z_i^{(j)}(d,T_v(t),0)$, we have found (\ref{Hsmall_inclusion_generation_inequality}) for $H_{small}=0$.
\end{proof}

\begin{remark}
     In the homogeneous case of only one class ($\beta_{ij}=\beta$, $k_{ij}=k$) and zero external field ("diluted Curie-Weiss"), Lemma \ref{lemma existence fixed point H_small H_big} provides a sufficient condition for the existence of at least one strictly positive solution if we set $H_{small}=\epsilon <<1$, $\epsilon>0$: the condition (\ref{condition_H_small}) reads 
     $$(k-1) F_\beta(\epsilon) \geq \epsilon $$
     which expanded around zero gives
     $$(k-1) F'_\beta(0)\epsilon \geq \epsilon $$
     and so  $F'_\beta(0) \geq \frac{1}{k-1}$, considering that $F'_\beta(0) = \tanh{(\beta)}$ the condition becomes 
     $$\beta \geq \tanh^{-1}\bigg(\frac{1}{k-1}\bigg) := \beta^+_c$$
     from which we derive an upper bound of the critical inverse temperature (a value of the inverse temperature after which the couple of ferromagnetic solutions is surely present). The upper bound actually coincides, in this case, with the critical value found by statistical physics calculations \cite{leone2002ferromagnetic}.
\end{remark}

    


==> trees/final_th.tex <==
\begin{theorem}
Consider an Ising model on a $k_{ij}$-regular tree $T_l$ of large depth $l$ with ferromagnetic couplings $\{\beta_{ij}\}$ and non-negative external fields $\{h_j\}$, for an arbitrary finite number of classes, i.e. $i,j = 1,...,n$. Consider, without loss of generality, that the root of the tree has external field $h_i$. The fixed point $\{\bar{z}_i^{(j)}\}_{i,j=1,...,n}$ with all positive entries of the $n^2$-dimensional recursion with $s=1,...,l-1$
$$z_i^{(j)} (s) = h_i + \sum_{k} (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(z_k^{(i)} (s-1)) \;\;\;\;\;\; \forall\;i,j = 1,...,n$$
exists, it is finite, unique, and it is achieved for any non-negative initial (boundary) condition. The corresponding equilibrium magnetization at the root of the tree is also positive and given by
$$m_i = \tanh\bigg( h_i + \sum_{k} k_{ik} F_{\beta_{ik}}(\bar{z}_k^{(i)}) \bigg)$$
where $F_\beta(x) = \tanh^{-1}\bigg( \tanh(\beta) \tanh(x)\bigg)$.
\end{theorem}

\begin{theorem}
Consider an Ising model on a $k_{ij}$-regular tree $T_l$ of large depth $l$ with ferromagnetic couplings $\{\beta_{ij}\}$ and any set of external fields $\{h_j\}$, for an arbitrary finite number of classes, i.e. $i,j = 1,...,n$. Consider, without loss of generality, that the root of the tree has external field $h_i$. If it exists $H\in \mbox{R}$ such that $H+h_i\geq 0\;\forall\;i=1,...,n$ and at the same time 
$$ \sum_{k} (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(H+h_k) > H   \;\;\;\;\;\; \forall\;i,j = 1,...,n$$
then the fixed point $\{\bar{z}_i^{(j)}\}_{i,j=1,...,n}$ with all positive entries and bounded by $\bar{z}_i^{(j)} \in [h_i+H,\infty)$ of the $n^2$-dimensional recursion with $s=1,...,l-1$
$$z_i^{(j)} (s) = h_i + \sum_{k} (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(z_k^{(i)} (s-1)) \;\;\;\;\;\; \forall\;i,j = 1,...,n$$
exists, it is finite, unique, and it is achieved surely for initial (boundary) condition $z_k^{(i)} (0) \in [H+h_k,\infty)$. The corresponding equilibrium magnetization at the root of the tree is also positive and given by
$$m_i = \tanh\bigg( h_i + \sum_{k} k_{ik} F_{\beta_{ik}}(\bar{z}_k^{(i)}) \bigg)$$
where $F_\beta(x) = \tanh^{-1}\bigg( \tanh(\beta) \tanh(x)\bigg)$.
\end{theorem}


==> trees/uniqueness.tex <==
\begin{lemma}
    Considering a $\mathbf{k}$-regular tree $T_v(t)$, if $\;\;\forall \; i,j,d$
    \begin{equation}
        \frac{d^2 z_i^{(j)}(d,T_v(t),H)}{dH^2} \leq 0 \;\;\;\;\;\;\;\;\;\;\;\;\; H\in[H_{small},H_{big}] 
    \label{concavity_cond}
    \end{equation}
    with $H_{small},H_{big}$ satisfying strictly the inequalities (\ref{condition_H_small}) and (\ref{condition_H_big}) of Lemma \ref{lemma existence fixed point H_small H_big}, then for the corresponding fixed point
    \begin{equation}
        \bar{z}_i^{(j)}(H_{small}) = \bar{z}_i^{(j)}(H_{big}) := \bar{z}_i^{(j)}
    \label{uniqueness_equation}
    \end{equation}
    Moreover, consider any (potentially dishomogeneous) vector of added field at the boundary $\mathbf{H} = \{ H_b, \; b\in V_*\}$. If $H_b\in[H_{small},H_{big}] \;\; \forall \; b\in V_*$, then for any finite $d$
    \begin{equation}
        \lim_{t\rightarrow \infty} z_i^{(j)}(d,T_v(t),\mathbf{H}) = \bar{z}_i^{(j)}
    \label{uniqueness_approach_eq}
    \end{equation} 
\label{lemma_uniqueness}
\end{lemma}

\begin{proof}
    If condition (\ref{concavity_cond}) is satisfied, then $H \mapsto z_i^{(j)}(d,T_v(t),H)$ is concave in $H\in[H_{small},H_{big}]$. Recall that for a concave function $f(x)$ it holds that $\forall \; x_1,x_2$ in the interval
    $$f(cx_1+(1-c)x_2) \geq cf(x_1) + (1-c)f(x_2)\;\;\;\;\;\;\;\;\;\;c\in[0,1]$$
    thus 
    $$ f(x_1) - f(x_2) \leq \frac{1}{c} [f(cx_1+(1-c)x_2)-f(x_2)]$$
    Choosing $x_1=H_{big}, x_2=H_{small}$
    \begin{equation}
        z_i^{(j)}(d,T_v(t),H_{big}) - z_i^{(j)}(d,T_v(t),H_{small}) \leq \frac{1}{c} [z_i^{(j)}(d,T_v(t),cH_{big}+(1-c)H_{small})-z_i^{(j)}(d,T_v(t),H_{small})]
    \label{consequence_concavity}
    \end{equation}
    for $c\in[0,1]$. Indicating with $ cH_{big}+(1-c)H_{small} := \Tilde{H}\in [H_{small},H_{big}]$, we look for 
    $$\Tilde{H}^*>H_{small} \;\; :\;\; z_i^{(j)}(d,T_v(t),\Tilde{H}^*) \leq  z_i^{(j)}(d,T_v(t+1),H_{small}) \quad \quad \forall \; i,j,d$$
    It exists surely if also
    $$z_i^{(j)}(t,T_v(t),\Tilde{H}^*)\leq z_i^{(j)}(t,T_v(t+1),H_{small}) \quad \quad \forall \; i,j$$
    which reads 
    $$\Tilde{H}^*\leq \sum_k (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(h_k+H_{small}) \quad \quad \forall \; i,j$$
    Recalling that $H_{small}$ is such that $H_{small}\leq \sum_k (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(h_k+H_{small}) $ and $\Tilde{H}^*>H_{small}$, then $H_{small} < \sum_k (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(h_k+H_{small})$ for all $i,j$ is a sufficient condition for the existence of $\Tilde{H}^*$, and we indicate the correspondent $c^*\in(0,1)$.\\
    Thus we can rewrite equation (\ref{consequence_concavity}) as
    \begin{equation}
        z_i^{(j)}(d,T_v(t),H_{big}) - z_i^{(j)}(d,T_v(t),H_{small}) \leq C [ z_i^{(j)}(d,T_v(t+1),H_{small})-z_i^{(j)}(d,T_v(t),H_{small})]
    \label{consequence_concavity_after H tilde}
    \end{equation}
    with $C = \frac{1}{c^*} = \frac{H_{big}-H_{small}}{\Tilde{H}- H_{small}}$ finite. \\
    Now we take the sum of the terms of (\ref{consequence_concavity_after H tilde}) over the depths of the tree, from $d$ to $t$ 
    \begin{equation}
        \sum_{l=d}^t z_i^{(j)}(d,T_v(l),H_{big}) - z_i^{(j)}(d,T_v(l),H_{small}) \leq C \bigg[\sum_{l=d}^t \bigg(z_i^{(j)}(d,T_v(l+1),H_{small})-z_i^{(j)}(d,T_v(l),H_{small})\bigg)\bigg]
    \label{sum_consequence_concavity_after H tilde}
    \end{equation}
    The l.h.s. is bounded inferiorly by $(t+1-d) [z_i^{(j)}(d,T_v(t),H_{big}) - z_i^{(j)}(d,T_v(t),H_{small})]$, as the smallest difference is the one at largest depth, for monotonicity arguments. On the other hand, for the r.h.s.
    \begin{align}
        &C \bigg[\sum_{l=d}^t \bigg(z_i^{(j)}(d,T_v(t+1),H_{small})-z_i^{(j)}(d,T_v(t),H_{small})\bigg)\bigg] =\\
        &= C [z_i^{(j)}(d,T_v(t+1),H_{small})-z_i^{(j)}(d,T_v(d),H_{small})\bigg]\leq \Tilde{C}
    \end{align}
    with $\Tilde{C}$ finite and independent of $t$. The equality is due to the fact that all other terms ($l\in[d+1,t]$) cancel out in the sum, while the upper bound is due to the boundedness of $z_i^{(j)}$ (Corollary \ref{corollary_boounds_and_monotony_H}).\\
    Thus, we can write
    $$(t+1-d) [z_i^{(j)}(d,T_v(t),H_{big}) - z_i^{(j)}(d,T_v(t),H_{small})] \leq \Tilde{C}$$
    $$ [z_i^{(j)}(d,T_v(t),H_{big}) - z_i^{(j)}(d,T_v(t),H_{small})] \leq \frac{\Tilde{C}}{(t+1-d)}$$
    Considering that the l.h.s. is always positive and taking the limit of large depth, we get
    $$\lim_{t\rightarrow\infty} [z_i^{(j)}(d,T_v(t),H_{big}) - z_i^{(j)}(d,T_v(t),H_{small})] := \bar{z}_i^{(j)}(H_{small}) - \bar{z}_i^{(j)}(H_{big}) = 0$$
    proving (\ref{uniqueness_equation}).
    \vskip 0.5 cm
    \noindent
    The second statement (\ref{uniqueness_approach_eq}) follows from the fact that, by the FKG inequalities, for $\;\;\forall \; i,j,d,v,t$,
    $$z_i^{(j)}(d,T_v(t),H_{small}) \leq z_i^{(j)}(d,T_v(t),\mathbf{H}) \leq z_i^{(j)}(d,T_v(t),H_{big})  $$
    if $H_b\in[H_{small},H_{big}] \;\; \forall \; b\in V_*$.     
\end{proof}
\vskip 1.5 cm
We are left to derive the conditions of validity of the concavity hypothesis, used in the previous Lemma.
\vskip 1.5 cm

\begin{lemma}
    If   $H_{small}\geq 0$ and 
    \begin{equation}
        h_i + H_{small} \geq 0 \;\;\;\;\;\;\; \forall \; i=1,...,n
    \label{positive_boundary}
    \end{equation}
    then 
    \begin{equation}
        \frac{d^2 z_i^{(j)}(d,T_v(t),H)}{dH^2} \leq 0 \;\;\;\;\;\;\;\;\;\;\;\;\; H\in[H_{small},H_{big}]
    \label{concavity_condition}
    \end{equation}
    with $H_{small},H_{big}$ satisfying respectively (\ref{condition_H_small}) and (\ref{condition_H_big}).
\label{lemma_concavity}
\end{lemma}

\begin{proof}
    We will use the expression of the first and second derivative of $F_\beta(x)$
    \begin{align}
        &\frac{\partial}{\partial x}\;F_\beta(x) = \frac{\sinh(2\beta)}{\cosh(2\beta)+\cosh(2x)} \;\geq 0\;\;\;\;\; \forall x \\
        &\frac{\partial ^2}{\partial x^2}\;F_\beta(x) = -\frac{2\sinh(2\beta)\sinh(2x)}{[\cosh(2\beta)+\cosh(2x)]^2} \;\leq 0\;\;\;\;\; \forall x\geq0
    \label{F_derivatives}
    \end{align}       
    We work directly on the recursion (\ref{recursion_regular_trees}), taking the second derivative with respect to the homogeneous field at the boundary
    \begin{align}
        \frac{d^2}{dH^2} z_i^{(j)}(d,T_v(t),H) &= \sum_k (k_{ik}-\delta_{jk}) \frac{d^2}{dH^2}F_{\beta_{ik}}(z_k^{(i)}(d+1,T_v(t),H)) =\\
        &= \sum_k (k_{ik}-\delta_{jk})  \frac{d}{dH}\bigg[\frac{\partial F_{\beta_{ik}}(z_k^{(i)}(d+1,T_v(t),H))}{\partial z_k^{(i)}(d+1,T_v(t),H)} \frac{d}{dH} z_i^{(j)}(d+1,T_v(t),H) \bigg] =\\
        &= \sum_k (k_{ik}-\delta_{jk}) \bigg[\frac{\partial^2F_{\beta_{ik}}(z_k^{(i)}(d+1,T_v(t),H))}{\partial z_k^{(i)}(d+1,T_v(t),H)^2} \bigg(\frac{d}{dH} z_i^{(j)}(d+1,T_v(t),H)\bigg)^2 +\\
        &+ \frac{\partial F_{\beta_{ik}}(z_k^{(i)}(d+1,T_v(t),H))}{\partial z_k^{(i)}(d+1,T_v(t),H)} \bigg(\frac{d^2}{dH^2} z_i^{(j)}(d+1,T_v(t),H)\bigg) \bigg]
    \label{rec_second_derivative}
    \end{align}
    so the derivatives are evaluated recursively, starting from the generation closest to the boundaries $d=t-1$, where
    $$
        \frac{d^2}{dH^2} z_i^{(j)}(t-1,T_v(t),H) = 
         \sum_k (k_{ik}-\delta_{jk}) \frac{\partial^2F_{\beta_{ik}}(z_k^{(i)}(t,T_v(t),H))}{\partial z_k^{(i)}(t,T_v(t),H)^2} \leq 0
    $$
    as $z_k^{(i)}(t,T_v(t),H)= h_k +H$. The last inequality follows from (\ref{F_derivatives}) and (\ref{positive_boundary}).\\
    Using the previous result  $\frac{d^2}{dH^2} z_i^{(j)}(t-1,T_v(t),H) \leq 0$ and the fact that for monotonicity $z_i^{(j)}(d,T_v(t),H)$ maintains non-negative anywhere, computing (\ref{rec_second_derivative}) for the second-last generation we get $\frac{d^2}{dH^2} z_i^{(j)}(t-2,T_v(t),H) \leq 0$, same for the third-last and so on. 
\end{proof}










%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%     COROLLARIES       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vskip 2 cm
\noindent
Now we list a series of corollaries that are the consequences of Lemmas \ref{lemma existence fixed point H_small H_big}, \ref{lemma_uniqueness} and \ref{lemma_concavity}, for different configurations of the fields associated to the classes, on trees.
\vskip 2 cm


\begin{corollary}
    For all positive fields, there exists exactly one fixed point of the recursion with all non-negative entries. Moreover, the latter fixed point is reached surely with any vector of added boundary fields $\mathbf{H}$ with all non-negative entries. 
\end{corollary}

\begin{proof}
    Fixing $H_{small}=0$ and $H_{big}=\infty$, for all positive fields the conditions (\ref{condition_H_small}) and (\ref{condition_H_big}) are all satisfied, and specifically $H_{small} < \sum_k (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(h_k+H_{small})$. Thus, the existence of at least one non-negative fixed point is a consequence of Lemma \ref{lemma existence fixed point H_small H_big} (or of Remark \ref{remark_proof_GKS}, using GKS). The concavity
    \begin{equation}
        \frac{d^2 z_i^{(j)}(d,T_v(t),H)}{dH^2} \leq 0 \;\;\;\;\;\;\;\;\;\;\;\;\; H\in[0,\infty) 
    \label{POSITIVE_concavity_cond}
    \end{equation}
    is guaranteed by Lemma \ref{lemma_concavity} , once noted that trivially $H_{small}+h_i>0\;\; \forall \; i=1,...,n$ . Thus, Lemma \ref{lemma_uniqueness} ensures the uniqueness of the latter fixed point, reached for any boundary added fields $\mathbf{H}$ with $H_b\in [0,\infty),\; b\in V_*$. Note that it is also the only non-negative fixed point, as trivially it is impossible to have fixed points with all non-negative entries with any $\bar{z}_i^{(j)}< h_i$ (see the recursion) and any other fixed point (all $\bar{z}_i^{(j)}\geq h_i$) corresponds to a choice of boundary fields $\mathbf{H}$ with $H_b\in [0,\infty),\; b\in V_*$.\\
    \\
    Note, alternatively, that for non-negative fields also the concavity (\ref{POSITIVE_concavity_cond}) can be proved using the correlation inequalities, specifically the GHS inequality: we write 
    \begin{align}
        \frac{d^2 z_i^{(j)}(d,T_v(t),H)}{dH^2} &= \frac{d}{dH} \bigg[ \frac{\partial z_i^{(j)}(d,T_v(t),H)}{\partial h'_l} \frac{dh'_l}{dH} \bigg] =\frac{d}{dH}  \frac{\partial z_i^{(j)}(d,T_v(t),H)}{\partial h'_l} = \\
        &= \frac{\partial^2 z_i^{(j)}(d,T_v(t),H)}{\partial h'_p \partial h'_l} \frac{dh'_p}{dH} = \frac{\partial^2 z_i^{(j)}(d,T_v(t),H)}{\partial h'_p \partial h'_l} \leq 0
    \label{GHS_POSITIVE_concavity_cond}
    \end{align}
    for any $l,p = 1,...,n$, indicating with $h'_{p/l} = h_{p/l} + H$. The last inequality follows from the GHS theorem, as the fields and couplings are all non-negative.    
\end{proof}

\vskip 2 cm

\begin{corollary}
    Consider all non-negative fields and at least one of them strictly positive. Moreover, for all the classes $i=1,...,n$ it must hold that $\sum_{j'} k_{ij'}\geq 2$, where $j'$ are the indices of the classes with a strictly positive associated field. There exists exactly one fixed point of the recursion with all positive entries. Moreover, the latter fixed point is reached surely with any added vector of boundary fields $\mathbf{H}$ with all non-negative entries. 
\end{corollary}

\begin{proof}
    Fixing $H_{small}=0$ and $H_{big}=\infty$, for all non-negative and at least one strictly positive field the conditions (\ref{condition_H_small}) and (\ref{condition_H_big}) are all satisfied. Specifically, $H_{small} < \sum_k (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(h_k+H_{small})$ as $k_{ij}\geq2 \;\forall \; i,j$, as the r.h.s. is always strictly greater than zero if $\sum_{j'} k_{ij'}\geq 2$. The proof than continues as in the strictly positive case.
\end{proof}

\vskip 2 cm

\begin{corollary}
    Consider any field configuration. If there exists $H_{small}\geq0$ satisying $H_{small} < \sum_k (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(h_k+H_{small})$ and also $H_{small} + h_i \geq 0 \;\forall\;i=1,...,n$, then there exists at least one fixed point of the recursion with all non-negative entries, and particularly there exists exactly one fixed point with entries $\bar{z}_i^{(j)} \in [h_i+H_{small},h_i + \sum_k (k_{ik}-\delta_{jk}) \beta_{ik}] $. Moreover, the latter fixed point is reached surely with any added vector of boundary fields $\mathbf{H}$ with all entries $H_b\in[H_{small},\infty)$, $b\in V_*$. 
\end{corollary}

\begin{proof}
    The proof consists in an application of the previous Lemmas with $H_{big}=\infty$ , which always fulfills the condition of Lemma \ref{lemma existence fixed point H_small H_big}. Moreover, if  there exists $H_{small}\geq0$ satisying $H_{small} < \sum_k (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(h_k+H_{small})$ and also $H_{small} + h_i \geq 0 \;\forall\;i=1,...,n$, then the concavity (Lemma \ref{lemma_concavity}) is also assured, as the recursion starts from a non-negative point and it is non-decreasing. The uniqueness (Lemma \ref{lemma_uniqueness}) then follows. Last, the given bound is a consequence of Corollary \ref{corollary_boounds_and_monotony_H}.
\end{proof}

% \begin{corollary} PENSAVO FOSSE VERO, PER CALCOLARE HSMALL PIù EFFICIENTEMENTE, MA APPARENTEMENTE NON LO è.
%     Consider any field configuration. If it is verified that  
%     \begin{equation}
%         \sum_k (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(h_k) \geq 0        \;\;\;\;\;\;\;\;\; \forall\;i,j
%     \label{1_cond}
%     \end{equation}
%     then a $H_{small}$ satisying $H_{small} < \sum_k (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(h_k+H_{small})$ and also $H_{small} + h_i \geq 0 \;\forall\;i=1,...,n$ exists if and only if, defining $h_{min} := \min_{i=1,...,n} h_i$, it holds that
%     \begin{equation}
%         \sum_k (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(h_k-h_{min}) > -h_{min}        \;\;\;\;\;\;\;\;\; \forall\;i,j
%     \label{2_cond}
%     \end{equation}
%     Moreover, the lowest $H_{small}$ is $H_{small}= -h_{min}$.\\
%     The fulfillment of (\ref{1_cond}) and (\ref{2_cond}) is then a sufficient condition for the existence of a fixed point of the recursion with all non-negative entries (and its uniqueness in the range $\bar{z}_i^{(j)} \in [h_i-h_{min},h_i + \sum_k (k_{ik}-\delta_{jk}) \beta_{ik}] $). Moreover, the latter fixed point is reached surely with any added vector of boundary fields $\mathbf{H}$ with all entries $H_b\in[-h_{min},\infty)$, $b\in V_*$.
% \end{corollary}

% \begin{proof}
%     If all the fields are non-negative and at least one is positive, both (\ref{1_cond}) and (\ref{2_cond}) are satisfied (the r.h.s in (\ref{2_cond}) is negative and the l.h.s. is positive) and the existence and uniqueness, as in Corollary \ref{}, are confirmed. If the fields are positive and negative, $h_{min}<0$. We take the set of $n^2$ functions
%     \begin{equation}
%         f_i^{(j)}(H) = \sum_k (k_{ik}-\delta_{jk}) F_{\beta_{ik}}(h_k+ H)       \;\;\;\;\; H\in[0,\infty) \;\;\;\;\;\;\forall \;i,j
%     \label{function}
%     \end{equation}
%     and $g(H) = H$. We claim that if condition (\ref{1_cond}) is satisfied, it is sufficient to see whether the condition for the existence of $H_{small}$ is verified at $H_{small}=-h_{min} = -\min_{i=1,...,n} h_i>0$. This comes from the fact that $f_i^{(j)}(H)$ are monotonic non-decreasing in the whole range and concave in  $H\in[-h_{min} ,\infty)$. EH, COL FATTO CHE NON è CONCAVA SEMPRE NON RIESCO A DIRE NULLA
% \end{proof}





==> work_in_progress/criticalities.tex <==
\textbf{Criticalities and doubts}

\begin{itemize}
    % \item $\Tilde{H}^*$ and finiteness of $\frac{1}{c}$
    % \item derivatives in the concavity
    \item free energy derivation: lo posso fare anche solo con le derivate sui campi prendendo come reference point tutti campi infiniti?
\end{itemize}

==> work_in_progress/unicita_positivi_generale.tex <==
%se riuscissimo a mostrare che almeno per quelle condizioni la magnetizzazione nel grafo è fra i bounds h_i+|h_min|  (e infinito, ma questo lo abbiamo), avremmo svoltato

%IDEA: dovremmo mostrare che, in caso di magnetizzazione del grafo tutta positiva, ...

\begin{corollary}
    CONJECTURE
    Consider any field configuration. If a fixed point of the recursion with all non-negative entries exists, then it is unique (the only fixed point of this kind).
\end{corollary}

\begin{proof}
    If such fixed point exists, then there must exist a step in the recursion, i.e., a certain distance $d^*$ from the root, such that all $z_i^{(j)}(d^*)\geq 0$, e da lì in poi rimangono tutti positivi indefinitamente. Costruisco un'altra ricorsione che parte da lì a cui associo boundary conditions tali che recupero le $z_i^{(j)}(d^*)$, queste boundary conditions saranno in generale disomogenee, del tipo 
    $$z_i^{(j)}(t,T_v(t),H) = h_i + \alpha_i^{(j)} H \geq 0$$
    Con tutti gli $\alpha_i^{(j)}\geq0$, si vede facilmente che questa verifica la concavità. Come passare da concavità a unicità in questo caso più generale? E' possibile senza avere H.small (H.big) ? \\
    \\
    Da estendere per unicità delle soluzioni negative notando che esiste una soluzione tutt negativa se e solo se esiste una soluzione tutta positiva in un sistema con campi opposti!
\end{proof}


==> work_in_progress/where_to_work.tex <==
\textbf{Where to work next}

\begin{itemize}
    \item Correspondence btw recursion and belief-propagation: lo abbiamo fatto nel limite termodinamico, sarebbe interessante seguire gli step di DemboMontanari per risultati sulla convergenza di BP per un grafo finito.
    \item Abbiamo provato e riprovato a trovare una condizione (corrispettivo delle GKS) che selezionasse quale soluzione della ricorsione corrisponde alla misura di Gibbs (equilibrio). Prossimo lavoro: visto che dalle simulazioni si trova che il modello con dinamica di Glauber converge sempre ad una delle soluzioni della ricorsione (in base a initial conditions) si potrebbe :\\
    - studiare la dinamica a livello teorico (coinvolgendo Collet)\\
    - scrivere la Bethe free energy per ciascuna delle soluzioni della ricorsione e vedere, tramite simulazioni su un grafo non troppo grande N=200 (così posso prendere tempi ragionevoli), se effettivamente il metodo euristico di prendere la soluzione con Bethe free en minore ha senso oppure no. Potrebbero sorgere problemi per la convergenza o N troppo basso etc.
    
    \item Si potrebbe studiare analiticamente il sistema con higher order interactions, cioè anche un ferromagnetico omogeneo con solo K interaction, per vedere come varia il phasespace.

    \item Si potrebbe vedere quanto la predizione è robusta rispetto a triadic closure, mi aspetto non molto. 

    \item ADJ SEPT 23: easy work con nuove disuguaglianze correlazione sugli alberi, applicazione su +h -h upper bound temperatura critica (congettura, non sappiamo passare dall'albero al grafo) corroborata da simulazioni glauber
\end{itemize}



